Momentum Particle Maximum Likelihood

Maximum likelihood estimation (MLE) of latent variable models is often recast as the minimization of a free energy functional over an extended space of parameters and probability distributions. This perspective was recently combined with insights from optimal transport to obtain novel particle-based algorithms for fitting latent variable models to data. Drawing inspiration from prior works which interpret `momentum-enriched' optimization algorithms as discretizations of ordinary differential equations, we propose an analogous dynamical-systems-inspired approach to minimizing the free energy functional. The result is a dynamical system that blends elements of Nesterov's Accelerated Gradient method, the underdamped Langevin diffusion, and particle methods. Under suitable assumptions, we prove that the continuous-time system minimizes the functional. By discretizing the system, we obtain a practical algorithm for MLE in latent variable models. The algorithm outperforms existing particle methods in numerical experiments and compares favourably with other MLE algorithms.

==> unused/convergence_old.tex <==
\section{Convergence Proofs}

We structure this section as follows:

\textbf{Notation}. We write $A \succeq B$ if $A-B$ is a positive semi-definite matrix. We define $\mathcal{M}$ and $\mathcal{M}'$

\subsection{Assumptions}

\textbf{Assumptions 1 (Log-Sobolev Inequality).} We shall assume that there exists some $C>0$, such that we have\adam{Need to define $\mathcal{M}$: presumably the product of the parameter space and the manifold(ish) of probabilities being considered?}
\begin{equation*}
    F\left(\theta, q\right)+\log p_{\theta^{*}}\left(y\right) \le \frac{1}{2C} \|\nabla_\mathcal{M} F(\theta, q)\|^2_{(\theta, q)} , \quad \forall (\theta, q) \in \mathcal{M},
    \label{eq:ls}
\end{equation*}
where the norm is given by
$$\|\nabla_\mathcal{M} F(\theta, q)\|^2_{(\theta, q)} = \|\nabla_\theta  F(\theta, q)\|^2 + \mathbb{E}_q \left \|\nabla_x \log \frac{q(X)}{p(y,X)}\right \|^2_2.$$ 
Given that a log-Sobolev inequality holds for $F((\theta,m), q)$, we show in the following proposition that a corresponding log-Sobolev inequality also holds for $F^{aug}(\theta, q)$.
%
\begin{proposition}
If $F(\theta, q)$ satisfies Assumption 1 with constant $C'$, then we have\adam{Need to define $\mathcal{M}'$}
$$
F^{aug}\left(z\right)+\log p_{\theta^{*}}\left(y\right) \le \frac{1}{2C} \|\nabla_{\mathcal{M}'} F^{aug}(z)\|^2_z, \quad \forall z:= ((\theta,m), q) \in \mathcal{M}',
$$
where $\frac{1}{2C} = \max\{\frac{1}{2C'}, \frac{1}{2\eta_\theta}, \frac{1}{2\eta_x}\}$ and the norm is defined as:
$$
\|\nabla_{\mathcal{M}'} F^{aug}(z)\|^2_z = \mathbb{E}_{q(m')}\|\nabla_\theta  F(\theta, q(\cdot |m') )\|^2 + \|\eta_\theta m\|_2^2+ \mathbb{E}_q \left \|\nabla_{(x,m')} \frac{\delta F^{aug}}{\delta q}(X, M') \right \|^2_2,
$$
where $q(m')$ is the marginal distribution of $q(x,m')$.
\end{proposition}

\adaml{We need to be clear what expectations are \emph{over}; various conventions exist but using captial letters for the random variables being integrated is one sensible option.}
\begin{proof}First notice that
\begin{align}
    \mathbb{E}_q \left \|\nabla_{(x,m')} \frac{\delta F^{aug}}{\delta q}(X,M')\right \|^2_2 &= \mathbb{E}_q \left \|\nabla_{(x,m')} \log \frac{q(X,M')}{p(y,X,M')}\right \|^2_2 \nonumber \\
    &= \mathbb{E}_q \left \|\nabla_x \log \frac{q(X,M')}{p(y,X)}\right \|^2_2 + \mathbb{E}_q \left \|\nabla_{m'} \log \frac{q(X,M')}{p(M')}\right \|^2_2 \nonumber \\
    &= \mathbb{E}_q \left \|\nabla_x \log \frac{q(X|M')}{p(y,X)}\right \|^2_2 + \mathbb{E}_q \left \|\nabla_{m'} \log \frac{q(M'|X)}{p(M')}\right \|^2_2. \label{eq:ls_inq_line}
\end{align}
Recall that $p(m') = \mathcal{N}(0, \frac{1}{\eta_x}I)$ which satisfies the log-Sobolev inequality with constant $\eta_x$, i.e., for any $q \in \mathcal{P}(\mathcal{X})$, we have
$
\mathrm{KL}(q|p) \le \frac{1}{2\eta_x} \mathbb{E}_q \left [ \nabla_{m'} \log \frac{q(M')}{p(M')}\right ].
$ Then, applying the log-Sobolev property to Eq.\ \ref{eq:ls_inq_line} for the conditional distribution $ q(\cdot|x)$, we obtain 
\begin{align}
    \mathbb{E}_q \left \|\nabla_{(x,m')} \frac{\delta F^{aug}}{\delta q} (X,M')\right \|^2_2 &\ge \mathbb{E}_q \left \|\nabla_x \log \frac{q(X|M')}{p(y,X)}\right \|^2_2 + 2\eta_x \mathbb{E}_{q(x)}\mathrm{KL}(q(m'|X)|p(m')). \label{eq:lsineq_1}
\end{align}
where $q(x)$ is the marginal distribution of $q(x,m')$.
\adaml{Perhaps this is obvious to the initiated\dots but how? Also, are there some typos? ($m$ for $m'$? is the $q(x)$ in the expectation subscript different in meaning to $q$ used elsewhere [I'd suggest $q(\cdot|x)$ if you want to indicate conditioning]?)}. Then, we have\adaml{Final $\nabla$ in line 1 should be $\nabla_{(x,m')}$, no? I'm struggling to quite recover the second line here, but I think I'm getting lost in notation.}
\begin{align*}
\frac{1}{2C} \|\nabla_{\mathcal{M}'} F^{aug}(z)\|^2_z &\ge \frac{1}{2C'} \mathbb{E}_{q(m')}\|\nabla_\theta  F(\theta, q(\cdot|M') )\|^2 + \frac{1}{2\eta_\theta}\|\eta_\theta m\|_2^2
\\
&+ \frac{1}{2C}\mathbb{E}_q \left \|\nabla_{(x,m')} \frac{\delta F^{aug}}{\delta q}(X,M')\right \|^2_2
\end{align*}
Applying the inequality of Eq.\ \ref{eq:lsineq_1}, we obtain 
\begin{align*}
\frac{1}{2C} \|\nabla_{\mathcal{M}'} F^{aug}(z)\|^2_z &\ge \frac{1}{2C'} \mathbb{E}_{q(m')}\|\nabla_\theta  F(\theta, q(\cdot |M') )\|^2 + \frac{1}{2\eta_\theta}\|\eta_\theta m\|_2^2
 \\
 &+ \frac{1}{2C} \mathbb{E}_q \left \|\nabla_x \log \frac{q(X|M')}{p(y,X)}\right \|^2_2 + \frac{\eta_x}{C} \mathbb{E}_{q(x)}\mathrm{KL}(q(m'|X)|p(m')).
\end{align*}
Since $\frac{1}{2C} \ge \frac{1}{2C'}$ and $\frac{\eta_x}{C} \ge 1$, we obtain
\begin{align*}
\frac{1}{2C} \|\nabla_{\mathcal{M}'} F^{aug}(z)\|^2_z &\ge \frac{1}{2C'}\mathbb{E}_{q(m')} \|\nabla_\theta  F(\theta, q(\cdot |M') )\|^2 + \frac{1}{2\eta_\theta}\|\eta_\theta m\|_2^2
 \\
 &+ \frac{1}{2C'} \mathbb{E}_q \left \|\nabla_x \log \frac{q(X|M')}{p(y,X)}\right \|^2_2 +  \mathbb{E}_{q(x)}\mathrm{KL}(q(m'|X)|p(m')).
\end{align*}
Applying the Log-Sobolev assumption of $F$ for $q(\cdot |m')$, we obtain
\begin{align*}
 \frac{1}{2C} \|\nabla_{\mathcal{M}'} F^{aug}(z)\|^2_z &\ge \mathbb{E}_{q(m')} F(\theta, q(\cdot|M'))  + \mathbb{E}_{q(x)}\mathrm{KL}(q(m'|X)|p(m'))  + \frac{\eta_\theta}{2}\|m\|^2_2 \\
  &+ \log p_{\theta^*} (y)\\
 &\ge F^{aug}((\theta, m), q) + \mathrm{KL}(q(x,m')|q(m')q(x')) + \log p_{\theta^*}(y) \\
 &\ge F^{aug}((\theta, m), q)+ \log p_{\theta^*}(y).
\end{align*}
This concludes the proof.
\end{proof}
%
%\juanl{I think this is a fair bet, only I would have $F^{aug}$ in the norm instead of $F$ (adding an extra $\norm{\nabla_m F^{aug}((\theta,m),q)}^2$ into the mix, and also something involving the $m'$ component of $p_\theta(x,y,m')$). Just a guess tho.}
%
\textbf{Assumptions 2.} We shall assume that the potential $U(\theta, x) := -\log p_\theta (y, x)$ has a $L_g$-Lipschitz gradient as a function. In other words, we have
%
$$
\left \| \nabla_{(\theta, x)} U(\theta, x) - \nabla_{(\theta, x)} U(\theta', x') \right \| \le L_g \left( \|x - x' \| + \|\theta - \theta' \| \right ) .
$$
%\adam{This looks weird; I initially assumed you wanted something uniform in $\theta$, but this is much stronger if you have $\theta'$ in the second term.}
If we have that $U(\theta,x) \in C^2$ then, we have that the absolute value of the eigenvalues of  $\nabla_{(\theta, x)} \nabla_{(\theta, x)} U(\theta, x)$ is bounded above by $L_g$, and $-L_gI \preceq \nabla_{(\theta, x)} \nabla_{(\theta, x)} U(\theta, x) \preceq L_g I$.
\subsection{Proof Idea}
Consider the Lyapunov function:
%
\begin{align}
    \mathcal{L}((\theta, m), q) &:=F^{aug}\left(\left(\theta,m\right),q\right)+\log p_{\theta^{*}}\left(y\right)\\
    &+\mathbb{E}_{q}\left[\left\langle \nabla_{(x,m')} \frac{\delta F^{aug}}{\delta q}\left(x,m'\right),M\nabla_{(x,m')}\frac{\delta F^{aug}}{\delta q}\left(x,m'\right)\right\rangle \right]\\
    &+\left\langle \nabla_{(\theta,m)} F^{aug}\left(\left(\theta,m\right),q\right),M'\nabla_{(\theta,m)}F^{aug}\left(\left(\theta,m\right),q\right)\right\rangle,
\end{align}
where $M=\frac{1}{L_g}\begin{pmatrix}\frac{1}{4} I_{d_x \times d_x} & \frac{1}{2} I_{d_x \times d_x}\\
\frac{1}{2} I_{d_x \times d_x} & 2 I_{d_x \times d_x}
\end{pmatrix} \in \mathbb{R}^{d_x \times d_x}$ and $M'= \in \mathbb{R}^{d_\theta \times d_\theta}$.

\textbf{Proof Idea.} The proof idea is as follows:

\textbf{Step 1.} Show that the time derivative has the form
\begin{align*}
    \frac{d}{dt}\mathcal{L}((\theta_t, m_t), q_t) &\le - \left \langle \nabla F^{aug}((\theta_t,m_t), q_t), S \nabla F^{aug}((\theta_t,m_t), q_t) \right \rangle \\
    &- \mathbb{E}_{q_t} \left [ \left \langle \nabla\frac{\delta F^{aug}}{\delta q}\left(x,m'\right), S'\nabla\frac{\delta F^{aug}}{\delta q}\left(x,m'\right)\right \rangle \right ],
\end{align*}
where $S$ and $S'$ are positive definite matrices.

\jl{the constants here are not exact - just guesses right now.}
\textbf{Step 2.} Show that we have $S \succeq \frac{1}{5C}\left ( M +  CI \right)$ and $S' \succeq \frac{1}{5C}\left ( M' +  CI \right)$.

\textbf{Step 3.} Hence, we have 
\begin{align*}
    \frac{d}{dt}\mathcal{L}((\theta_t, m_t), q_t) &\le - \frac{1}{5C} \left (C\|\nabla F^{aug}((\theta_t,m_t), q_t)\|^2 +  \left \langle \nabla F^{aug}(\theta_t, q_t), M \nabla F^{aug}(\theta_t, q_t)\right \rangle \right ) \\ 
    &- \frac{1}{5C} \left (  C\mathbb{E}_{q_t}\|\nabla\frac{\delta F^{aug}}{\delta q}(x,m')\|^2_2  + \mathbb{E}_{q_t} \left [ \left \langle \nabla\frac{\delta F^{aug}}{\delta q}\left(x,m'\right), M'\nabla\frac{\delta F^{aug}}{\delta q}\left(x,m'\right)\right \rangle \right ] \right ) 
\end{align*}
\juanl{Should the third term in the above RHS be inside the first term in the RHS?}
Applying ``log-Sobolev'', we have as desired
$$
\frac{d}{dt}\mathcal{L}(\theta_t, q_t) \le - \frac{1}{5C} \mathcal{L}(\theta_t, q_t).
$$

\subsection{Step 1}
We can write the time derivative of the Lyapunov function $\mathcal{L}$ as
%
% \begin{align*}
% \frac{d}{dt}\mathcal{L}((\theta_t,\mu_t),q_t)=&\frac{d}{dt}F^{aug}((\theta_t,\mu_t),q_t)
% \end{align*}
%
\begin{align}
    \frac{d}{dt}\mathcal{L}\left(\left(\theta_{t},m_{t}\right),q_{t}\right)&= - \left\langle \nabla_{(\theta,m)}\mathcal{L}\left(\left(\theta_{t},m_{t}\right),q_{t}\right),\begin{pmatrix}0 & -I\\
I & \gamma_{\theta}I
\end{pmatrix}\nabla_{(\theta,m)} F_{q}^{aug}\left(\theta_{t},m_{t}\right)\right\rangle \label{eq:dldthetadt} \\
&-\mathbb{E}_{q_{t}}\left\langle \nabla_{(x,m')}\delta_{q_{t}}\mathcal{L}_{\theta}\left(x,m\right),\begin{pmatrix}0 & -I\\
I & \gamma_{\theta}I
\end{pmatrix}\nabla_{(x,m')}\delta_{q_{t}}F_{\theta_{t}}^{aug}\left(x_{t},m_{t}'\right)\right\rangle \label{eq:dldqdt}.
\end{align}
%
We treat the terms Eq.\ \ref{eq:dldthetadt} and Eq.\ \ref{eq:dldqdt} separately.

\textbf{Eq.\ \ref{eq:dldthetadt}}. We have
%
\begin{align}
    \text{Eq.\ \ref{eq:dldthetadt}}	&= - \left\langle \nabla_{\left(\theta,m\right)}F^{aug}\left(\left(\theta,m\right),q\right), \Gamma \nabla_{(\theta, m)}
F_{q}^{aug}\left(\theta_{t},m_{t}\right)\right\rangle \label{eq:dldthetadt_t1}\\
%
&-2\mathbb{E}_{q}\left[\left\langle \nabla_{(\theta,m)} \nabla_{(x,m')}\left[\delta_{q}F_{\theta_{t}}^{aug}\left(x,m\right)\right]M\nabla_{(x,m')}\left [\delta_{q}F_{\theta_{t}}^{aug}\left(x,m\right) \right ],\begin{pmatrix}0 & -I\\
I & \gamma_{\theta}I
\end{pmatrix}\nabla_{(\theta, m)}
F_{q}^{aug}\left(\theta_{t},m_{t}\right)\right\rangle \right]. \label{eq:dldthetadt_t2}
\end{align}
where $\Gamma =\left[I-2M'\nabla_{\left(\theta,m\right)}\nabla_{\left(\theta,m\right)}\left[F_{q}^{aug}\left(\theta,m\right)\right]\right]\begin{pmatrix}0 & -I\\
I & \gamma_{\theta}I
\end{pmatrix}$.
We can write Eq.\ \ref{eq:dldthetadt_t1} equivalently in terms of a \textit{symmetric} matrix $\Gamma^{sym}:=\frac{\Gamma + \Gamma^\top}{2}$. This is due to the fact that a square matrix $\Gamma$ can be decomposed into a sum of symmetric $\Gamma^{sym}$ and skew-symmetric $\Gamma^{skew}:=\frac{\Gamma - \Gamma^\top}{2}$ matrices, i.e., $\Gamma = \Gamma^{sym}+ \Gamma^{skew}$. We have that $\left \langle z, \Gamma z\right \rangle = \left \langle z, \Gamma^{sym} z\right \rangle$ as the skew-symmetric component does not play a role, i.e., $\left \langle z, \Gamma^{skew}z \right \rangle = 0$. Hence, Eq.\ \ref{eq:dldthetadt_t1} can be written equivalently as
$$
- \left\langle \nabla_{\left(\theta,m\right)}F^{aug}\left(\left(\theta,m\right),q\right), \Gamma^{sym} \nabla_{(\theta, m)}
F_{q}^{aug}\left(\theta_{t},m_{t}\right)\right\rangle,
$$
where 
$$
\Gamma^{sym} = \frac{1}{2}\begin{pmatrix}a\eta_{\theta} I  & -b\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+(\frac{a}{2}\eta_{\theta}\gamma_{\theta}+c\eta_{\theta}) I\\
-b\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+(\frac{a}{2}\eta_{\theta}\gamma_{\theta}+c\eta_{\theta}) I & - a\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+(2c\eta_{\theta} + 1)\gamma_{\theta}I
\end{pmatrix}.
$$

\textbf{Eq.\ \ref{eq:dldqdt}}. We introduce the function $h(x, m') := \sqrt{\frac{q(x,m')}{p_\theta(y,x,m')}}$ to simplify the notation. Note that we can write the first variation $\delta_{q_t} F^{aug}_\theta (x,m') = 2 \log h_\theta(x,m')$. Since, we have that the first variation $\delta_{q_{t}}\mathcal{L}_{\theta}\left(x,m\right)$ is
%
\begin{align*}
    \delta_{q_{t}}\mathcal{L}_{\theta}\left(x,m\right)&= 2\log h_\theta(x,m')  \\
    &+  \frac{4}{h_\theta(x,m')}  \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m') \\
    &-2\left \langle \nabla_{(\theta,m)} \log {p_{\theta}(y,x,m')}
, M \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right \rangle.
\end{align*}
%
The derivation is provided in Section \ref{sec:lyapunov_fv}. More specifically, the second term is given in Prop.\ \ref{prop:fv_L2}, and the third term in Prop.\ \ref{prop:fv_L1}. Thus, we have for Eq.\ \ref{eq:dldqdt} in the time derivative of the first variation 
%
\begin{align}
    \text{Eq.\ \ref{eq:dldqdt}} &= - 4\mathbb{E}_{q_t} \left \langle  \nabla_{(x,m')} \log h_\theta(x,m') , \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle \label{eq:dldqdt_t1}\\
&- 8\mathbb{E}_{q_t} \left \langle \nabla_{(x,m')} \left ( \frac{1}{h_\theta(x,m')}  \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')\right ), \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle \label{eq:dldqdt_t2} \\
&- 4 \mathbb{E}_{q_t} \left \langle \nabla_{(x,m')}\left \langle \nabla_{(\theta,m)} \log {p_{\theta}(y,x,m')}
, M' \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right \rangle,\begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle. \label{eq:dldqdt_t3}
\end{align}
%
For the first term, i.e., Eq.\  \ref{eq:dldqdt_t1}, we have
$$
\text{Eq.\  \ref{eq:dldqdt_t1}} = -4\gamma_x \|\nabla_m' \log h_\theta (x,m')\|^2 = - \gamma_x \mathbb{E}_{q_t} \left \|\nabla_{m'}\log \left (\frac{q(x, m')}{p_\theta (y,x,m')} \right ) \right \|^2.
$$
For the second term, i.e., Eq.\  \ref{eq:dldqdt_t2}, we have
%
\begin{align*}
    \text{Eq.\  \ref{eq:dldqdt_t2}} =  &- 2\gamma_x \mathbb{E}_{q_t} \left \langle \nabla_{x,m'}\nabla_{m'} \log \left ( \frac{q(x,m')}{p(y,x, m')} \right ),
 M\nabla_{x,m'}\nabla_{m'}\log \left ( \frac{q(x,m')}{p(y,x, m')} \right ) \right \rangle_F \\
- &\mathbb{E}_{q_t} \left \langle \nabla_{(x,m')}\log \left ( \frac{q(x,m')}{p(y,x, m')} \right ),T\nabla_{(x,m')}\log \left ( \frac{q(x,m')}{p(y,x, m')} \right ) \right \rangle 
\end{align*}
%
where $$
%
T = \frac{1}{2}\begin{pmatrix}
    a\eta_x I & \left ( \left [ c\eta_x +  a\gamma_x \eta_x \right ]  I + b \mathrm{Hess}_x [\log p_\theta (y,x)] \right )\\
    \left ( \left [ c\eta_x +  a\gamma_x \eta_x \right ]  I + b \mathrm{Hess}_x [\log p_\theta (y,x)] \right ) &   4\gamma_x c\eta_x I + {a}\mathrm{Hess}_x[\log p_\theta (y,x)]
\end{pmatrix}.
$$
%
The derivation can be found in Section \ref{sec:dldqdt_t2}. We can combine Line \ref{eq:dldqdt_t1} with the second term of Line \ref{eq:dldqdt_t2} to obtain 
%
$$
\text{Line \ref{eq:dldqdt_t1}} + \text{Line \ref{eq:dldqdt_t2}} = -  8 \gamma_x \bar{\mathbb{E}}_\theta \left \langle \nabla_{x,m'}\nabla_{m'}h,
 M\nabla_{x,m'}\nabla_{m'}h \right \rangle_F - 4\bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')}h,T'\nabla_{(x,m')}h\right \rangle.
$$
%
where $T' = T + \begin{bmatrix}
    0 & 0 \\
    0 & \gamma_x
\end{bmatrix}$.

\textbf{Cross Terms.} We will now deal with the cross terms, i.e., Eq.\ \ref{eq:dldqdt_t3} and \ref{eq:dldthetadt_t2}. In Section \ref{sec:xterm}, we show that we have the following upper-bound: 
$$
\text{Eq.\ \ref{eq:dldqdt_t3}} + \text{Eq.\ \ref{eq:dldthetadt_t2}} \le L_{g}b
 \left[\left\Vert \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right\Vert ^{2}+\mathbb{E}_{q_t} \left\Vert \nabla_{(x,m')} \delta_{q}F_{\theta_{t}}^{aug}(x,m')\right\Vert ^{2}\right]
$$
Hence, we have shown that 
\begin{align*}
    \frac{d}{dt}\mathcal{L}((\theta_t, m_t), q_t) &\le - \left \langle \nabla F^{aug}_{q_t}(\theta_t,m_t), S \nabla F^{aug}_{q_t}(\theta_t,m_t) \right \rangle \\
    &- \mathbb{E}_{q_t} \left [ \left \langle \nabla\frac{\delta F^{aug}}{\delta q}\left(x,m'\right), S'\nabla\frac{\delta F^{aug}}{\delta q}\left(x,m'\right)\right \rangle \right ],
\end{align*}
where $S = \Gamma_{sym} - \frac{L_g b}{2} I$, and $S' = T-\frac{L_gb}{2} I$.
\subsection{Step 2}

We want to show that $S \succeq K(M + CI)$ and $S' \succeq K(M + CI)$.

We begin with showing that $S \succeq K(M + CI)$. This is equivalent to showing that
$$
S-K(M + CI) =
\begin{pmatrix}\alpha I   
& -\frac{b}{2}\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+ \beta I \\
-\frac{b}{2}\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+\beta I & - \frac{a}{2}\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+\kappa I
\end{pmatrix} 
$$
where the constants  are
\begin{align*}
    \alpha &:= \frac{1}{2}(a\eta_{\theta} - 2(K(b + C) + L_gb)) \\
    \beta &:= \frac{1}{2}\left (\left (\frac{a}{2}\gamma_{\theta}+c \right )\eta_{\theta} - aK \right ) \\
    \kappa &:= \frac{1}{2}((2c\eta_{\theta} + 1)\gamma_{\theta} - 2(K(C + c) +L_gb) )
\end{align*}
is a p.s.d. matrix. We will show this by showing the eigenvalues are non-negative. The characteristic equation is given by
\begin{align*}
    \mathrm{det}(S-K(M+CI) - l I) &= \mathrm{det}\begin{pmatrix}(\alpha - l) I   
& -\frac{b}{2}\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+ \beta I \\
-\frac{b}{2}\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+\beta I & - \frac{a}{2}\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+(\kappa- l) I
\end{pmatrix} \\
&=\mathrm{det}\left ( (\alpha  - l)(\kappa - l) I - (\alpha - l)\frac{a}{2}\nabla_{\theta}\nabla_{\theta}F_{q} -  \left (-\frac{b}{2}\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+\beta I \right )^2 \right ) = 0,
\end{align*}
where for the last line we use the fact that $\frac{a}{2}\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+(\kappa- l) I$ and $-\frac{b}{2}\nabla_{\theta}\nabla_{\theta}F_{q}\left(\theta\right)+ \beta I$ commute.

Denote $\nabla_\theta \nabla_\theta F_q (\theta) = U\Lambda U^\top$ be its eigenvalue decomposition. Note that since $0 \preceq \nabla\nabla U_\theta (y,x) \preceq L_gI$, we have $ 0 \preceq \nabla_\theta \nabla_\theta F_q (\theta) \preceq L_g I $.
Hence, we have
%
\begin{align*}
    \mathrm{det}(S-K(M+CI) - l I) &= \mathrm{det}\left (U \left (  (\alpha -l)(\kappa - l)I - \frac{a}{2}(\alpha - l)\Lambda -\left (- \frac{b}{2}\Lambda + \beta I\right )^2\right ) U^\top \right ) = 0.
\end{align*}
Since the determinant is equal to the product of the eigenvalues, we require all eigenvalues of the above matrix to be zero. Hence, we require that  
\begin{align*}
    l^2 + \left ( \frac{a}{2} \lambda -\alpha -\kappa\right ) l - \left (\frac{b^2}{4} \lambda^2 +\left ( \frac{\alpha a}{2}- b\beta\right ) \lambda - \alpha \kappa + \beta^2  \right ) = 0 
\end{align*}
%
In order to ensure that the eigenvalues are positive $l$, we require that
\begin{align*}
    &\frac{a}{2} \lambda -\alpha -\kappa \le 0,  \\
    &\frac{b^2}{4} \lambda^2 +\left ( \frac{\alpha a}{2}- b\beta\right ) \lambda - \alpha \kappa +\beta^2    \le 0,
\end{align*}
for all $\lambda \in [0, L_g]$. Since $\frac{a}{2} \lambda -a-\kappa \le 0$ is strictly increasing in $\lambda$, and $\frac{b^2}{4} \lambda^2 +\left ( \frac{\alpha a}{2}- b\beta\right ) \lambda - \alpha \kappa$ is a quadratic function, it is sufficient to ensure that the inequalities are satisfied at the end-points of $\lambda$. In order words, we require
\begin{align*}
    &\frac{a}{2} L_g -\alpha -\kappa \le 0,  \\
    &\frac{b^2}{4} L_g^2 +\left ( \frac{\alpha a}{2}- b\beta\right ) L_g - \alpha \kappa +\beta^2   \le 0, \\
    &\frac{b^2}{4} L_g^2 - \alpha \kappa  + \beta^2   \le 0.
\end{align*}
Under our assumptions, we have $\alpha = $ 

\subsection{Step 3}

\subsection{Supporting Proofs and Derivations}

\textbf{Notation}. We write $\bar{\mathbb{E}}_\theta [f]$ to denote the functional defined as
$$
\bar{\mathbb{E}}_\theta [f] := \int p_\theta(y, x, m') f(x,m')dxdm'
$$

\subsubsection{First Variation of $\mathcal{L}$}
\label{sec:lyapunov_fv}
In order to calculate the time derivative of $\mathcal{L}$, we require the first variation of $\mathcal{L}$. We have
$$
\delta_{q_t} \mathcal{L} = \delta_{q_t} F^{aug}_\theta + \delta_{q_t} \mathcal{L}^{(1)}_\theta + \delta_{q_t} \mathcal{L}^{(2)}_\theta,
$$
where 
\begin{align*}
\mathcal{L}^{(1)}_\theta &:q\mapsto \mathbb{E}_{q}\left\langle \nabla_{(x,m')} \delta_{q}F_{\theta}^{aug}\left(x,m'\right),M\nabla_{(x,m')} \delta_{q}F_{\theta}^{aug}\left(x,m'\right)\right\rangle \\
\mathcal{L}^{(2)}_\theta &:q\mapsto \left\langle \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right),M'\nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right\rangle.
\end{align*}

For the first variation of $\mathcal{L}^{(1)}_\theta$, we have the following result:

\begin{proposition}
\label{prop:fv_L1}
The first variation of $\mathcal{L}^{(1)}_\theta$ is given by
    $$
    \delta_{q_t}\mathcal{L}^{(1)}_\theta (x,m') = \frac{4}{h_\theta(x,m')}  \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m'),
    $$
    where $h_\theta(x, m') := \sqrt{\frac{q(x,m')}{p_\theta(y,x,m')}}$ and the operator $\left (\nabla_{(x,m')} \right )^*$ is given as $$\left (\nabla_{(x,m')} \right )^*(f)(x,m'):= - \nabla_{(x,m')}  \log p_\theta(y,x,m') \cdot f(x,m') - \nabla_{(x,m')} \cdot  f(x,m'),$$
    where $\nabla_{x}\cdot$ is the divergence operator w.r.t. $x$.
\end{proposition}
\begin{proof}
To simplify the notation, we omit all subscripts for the gradient and divergent operators as they are all taken with respect to $(x,m')$.

We can write $\mathcal{L}^{(1)}$ equivalently as
    $$
    \mathcal{L}^{(1)}_\theta :q\mapsto 4\int \left\langle \nabla_{(x,m')} \sqrt{\frac{q(x,m')}{p_\theta(y,x,m')}},M\nabla_{(x,m')} \sqrt{\frac{q(x,m')}{p_\theta(y,x,m')}}\right\rangle p_\theta(y,x,m')dxdm'.
    $$
    Then, using the fact that
$$
\sqrt{\frac{q+\epsilon \chi (x,m')}{p_\theta(y,x,m')}} = \sqrt{\frac{q(x,m')}{p_\theta(y,x,m')}} + \epsilon \frac{\chi(x,m')}{2\sqrt{q(x,m')p_\theta(y,x,m')}} + o(\epsilon),
$$
we can calculate the first variation using the definition 
\begin{align*}
    \lim_{\epsilon\rightarrow 0} \frac{\mathcal{L}^{(1)}_\theta (q+\epsilon \chi)- \mathcal{L}^{(1)}_\theta(q)}{\epsilon} &= 4\int \left\langle \nabla  \left(\frac{\chi(x,m')}{\sqrt{q(x,m')p_\theta(y,x,m')}} \right ),M\nabla \sqrt{\frac{q(x,m')}{p_\theta(y,x,m')}}\right\rangle p_\theta(y,x,m')dxdm' \\
    &= -4\int \frac{\chi(x,m')}{\sqrt{q(x,m')p_\theta(y,x,m')}}  \nabla \cdot \left(p_\theta(y,x,m') M\nabla \sqrt{\frac{q(x,m')}{p_\theta(y,x,m')}}  \right )dxdm',
\end{align*}
where the last line is obtained using integration by parts. Hence, we can identify the first variation as
$$
- \frac{4}{\sqrt{q(x,m')p_\theta(y,x,m')}}  \nabla \cdot \left(p_\theta(y,x,m') M\nabla \sqrt{\frac{q(x,m')}{p_\theta(y,x,m')}}  \right ).
$$
Finally, we can rewrite this in terms of the function $h_\theta(x, m') := \sqrt{\frac{q(x,m')}{p_\theta(y,x,m')}}$ to obtain
\begin{align*}
    - \frac{4}{h_\theta(x,m')}  \left [ \nabla  \log p_\theta(y,x,m') \cdot \left ( M\nabla h_\theta(x,m')  \right ) +\nabla\cdot \left( M\nabla h_\theta(x,m')  \right ) \right  ].
\end{align*}
This follows by expanding the divergences and using some log rules.
\end{proof}
\jl{What happens when $v$ is a matrix?}
The operator $\left (\nabla_{(x,m')} \right )^*$ is actually the adjoint operator of $\nabla$ w.r.t.\ to the inner product $\bar{\mathbb{E}}_\theta \left [\langle \cdot , \cdot\rangle \right ]$. In other words, we have that
\begin{align*}
    \bar{\mathbb{E}}_\theta \langle \nabla_{(x,m')} f(x,m'), v(x,m')\rangle &= - \int  f(x,m') \nabla_{(x,m')} \cdot ( p(y,x,m')v(x,m'))dxdm' \\
    &=- \bar{\mathbb{E}}_\theta \left [ f(x,m') \left ( \nabla_{(x,m')} \log p(y,x,m')\cdot v(x,m') \right ) \right ]\\
    &- \bar{\mathbb{E}}_\theta \left [ f(x,m') \left ( \nabla_{(x,m')} \cdot v(x,m') \right )  \right ]\\
    &=\bar{\mathbb{E}}_\theta\left [  f(x,m') \left (\nabla_{(x,m')} \right )^* (v)(x,m') \right ]
\end{align*}
where we use integral by parts in the first line. Note that this applies to operators $\left (\nabla_{x} \right )^*$ and $\left (\nabla_{(x,m')} \right )^*$ where the divergences and gradients are taken w.r.t $x$ and $m'$.

As for the second first variation $\delta_q \mathcal{L}^{(2)}_\theta$, we have the following:
\begin{proposition}
\label{prop:fv_L2}
The first variation of the functional $\delta_{q_t} \mathcal{L}^{(2)}_\theta$ is given by
$$
\delta_q \mathcal{L}^{(2)}_\theta (x,m') = -2\left \langle \nabla_{(\theta,m)} \log {p_{\theta}(y,x,m')}
, M' \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right \rangle.
$$    
\end{proposition}
\begin{proof}
First note that we have
$$
\nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right) = \begin{pmatrix}-\int\nabla_{\theta}{\log p_{\theta}(y,x,m')}q(dx,dm')\\
\eta_{\theta}m
\end{pmatrix}
$$
Then, we have
$$
\nabla_{(\theta,m)} F_{q+\epsilon \chi }^{aug}\left(\theta,m\right) = \nabla F_{q}^{aug}\left(\theta,m\right) - \epsilon \begin{pmatrix}\int \nabla_{\theta} \log {p_{\theta}(y,x,m')}\chi (x,m')dxdm'\\
0
\end{pmatrix}.
$$
Hence, we have
\begin{align*}
\lim_{\epsilon \rightarrow 0}\frac{\mathcal{L}^{(2)}(q+\epsilon \chi) - \mathcal{L}^{(2)}(q)}{\epsilon} =  - \int  2\left \langle \begin{pmatrix}\nabla_{\theta} \log {p_{\theta}(y,x,m')}\\
0
\end{pmatrix}
, M' \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right \rangle \chi(x,m')dxdm'.
\end{align*}
Hence, the first variation is given by
$$
-2\left \langle \nabla_{(\theta,m)} \log {p_{\theta}(y,x,m')}
, M' \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right \rangle.
$$
\end{proof}

\begin{proposition}   
\end{proposition}
\subsubsection{Simplifying Eq.\  \ref{eq:dldqdt_t2}}
\label{sec:dldqdt_t2}
From the quotient rule, we have 
\begin{align*}
    &\nabla_{(x,m')} \left ( \frac{1}{h_\theta(x,m')}  \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')\right ) \\
    = &\frac{\nabla_{(x,m')} \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')}{h_\theta(x,m')} \\
    - &\frac{\nabla_{(x,m')} h_\theta(x,m')  \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')}{h_\theta(x,m')^2}
\end{align*}
Then, we can write Eq.\  \ref{eq:dldqdt_t2} as 
\begin{align}
&- 8 \mathbb{E}_{q_t} \left \langle \nabla_{(x,m')} \left ( \frac{1}{h_\theta(x,m')}  \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')\right ), \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle  \nonumber  \\ 
&= - 8 
\mathbb{E}_{q_t} \left \langle \frac{\nabla_{(x,m')} \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')}{h_\theta(x,m')}, \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle  \label{eq:quotient_t1}\\
&+ 8 \mathbb{E}_{q_t} \left \langle \frac{\nabla_{(x,m')} h_\theta(x,m')  \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')}{h_\theta(x,m')^2}, \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle \label{eq:quotient_t2}
\end{align}
%
We can simplify the terms individually, whose reduction can be found in ... Hence,  we can write Eq.\ \ref{eq:dldqdt_t2} equivalently the following:
\begin{align}
    &=  16\gamma_{x}\bar{\mathbb{E}}_\theta \left\langle \nabla_{(x,m')}\nabla_{m'}h_{\theta}(x,m'),M\frac{\nabla_{(x,m')} h_{\theta}(x,m')}{h_{\theta}(x,m')}\otimes\nabla_{m'} h_{\theta}(x,m')\right\rangle _{F}\label{eq:g_t1}\\
 %
	&- 8\gamma_{x}\bar{\mathbb{E}}_\theta \left\langle \frac{\nabla_{(x,m')}h_{\theta}(x,m')}{h_{\theta}(x,m')}\otimes\nabla_{m'}h_{\theta}(x,m'),M\frac{\nabla_{(x,m')}h_{\theta}(x,m')}{h_{\theta}(x,m')}\otimes\nabla_{m'}h_{\theta}(x,m')\right\rangle_F \label{eq:g_t2}\\
 &- 8\gamma_x \bar{\mathbb{E}}_\theta \left \langle \nabla_{x,m'}\nabla_{m'}h(x,m'),M\nabla_{x,m'}\nabla_{m'}h(x,m') \right \rangle_F\label{eq:g_t3}\\
&-  2a\eta_x\mathbb{E}_\theta [\|\nabla_x h(x,m')\|^2_2 \label{eq:g_t4}\\
&- 4 \bar{\mathbb{E}}_\theta \left \langle \nabla_{x} h_\theta (x,m'), \left ( \left [ c\eta_x +  a\gamma_x \eta_x \right ]  I + b \mathrm{Hess}_x [\log p_\theta (y,x)] \right ) \nabla_{m'} h (x,m') \right \rangle \label{eq:g_t5}\\
&- 8\bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} h_\theta (x,m'), \left ( c\eta_x\gamma_x I + \frac{a}{4}\mathrm{Hess}_x[\log p_\theta (y,x)] \right ) \nabla_{m'} h_\theta (x,m')\right \rangle.\label{eq:g_t6}
\end{align}
We can rewrite the sum of Eq.\ \ref{eq:g_t1}, \ref{eq:g_t2}, \ref{eq:g_t3} as
\begin{align*}
&-8\gamma_x \bar{\mathbb{E}}_\theta \left \langle \nabla_{x,m'}\nabla_{m'}h(x,m'),M\nabla_{x,m'}\nabla_{m'}h(x,m') \right \rangle_F \\
    & +16\gamma_{x}\bar{\mathbb{E}}_\theta \left\langle \nabla_{(x,m')}\nabla_{m'}h_{\theta}(x,m'),M\frac{\nabla_{(x,m')} h_{\theta}(x,m')}{h_{\theta}(x,m')}\otimes\nabla_{m'} h_{\theta}(x,m')\right\rangle _{F}\\
 %
	&-8\gamma_{x}\bar{\mathbb{E}}_\theta \left\langle \frac{\nabla_{(x,m')}h_{\theta}(x,m')}{h_{\theta}(x,m')}\otimes\nabla_{m'}h_{\theta}(x,m'),M\frac{\nabla_{(x,m')}h_{\theta}(x,m')}{h_{\theta}(x,m')}\otimes\nabla_{m'}h_{\theta}(x,m')\right\rangle_F\\
 &= -8\gamma_x \bar{\mathbb{E}}_\theta \left \langle \nabla_{x,m'}\nabla_{m'}h - \frac{\nabla_{(x,m')}h_{\theta}}{h_{\theta}}\otimes\nabla_{m'}h_{\theta}(x,m'),
 M\left (  \nabla_{x,m'}\nabla_{m'}h -\frac{\nabla_{(x,m')}h_{\theta}}{h_{\theta}}\otimes\nabla_{m'}h_{\theta}\right) \right \rangle_F.
\end{align*}
Since we have that $\partial_x \partial_m h = \partial_x (h \partial_m \log h) = (\partial_x h) (\partial_m \log h) + h (\partial_x \partial_m \log h)$, we can write the above as
%
\begin{align*}
    & - 8 \gamma_x \bar{\mathbb{E}}_\theta \left \langle \nabla_{x,m'}\nabla_{m'}h - \frac{\nabla_{(x,m')}h_{\theta}}{h_{\theta}}\otimes\nabla_{m'}h_{\theta}(x,m'),
 M\left (  \nabla_{x,m'}\nabla_{m'}h -\frac{\nabla_{(x,m')}h_{\theta}}{h_{\theta}}\otimes\nabla_{m'}h_{\theta}\right) \right \rangle_F \\
 &= - 8\gamma_x \mathbb{E}_{q_t} \left \langle \nabla_{x,m'}\nabla_{m'} \log h,
 M\nabla_{x,m'}\nabla_{m'}\log h \right \rangle_F \\
 &= - 2\gamma_x \mathbb{E}_{q_t} \left \langle \nabla_{x,m'}\nabla_{m'} \log \left ( \frac{q(x,m')}{p(y,x, m')} \right ),
 M\nabla_{x,m'}\nabla_{m'}\log \left ( \frac{q(x,m')}{p(y,x, m')} \right ) \right \rangle_F
\end{align*}

As for the other terms, we can combine Eq.\ \ref{eq:g_t4}, Eq.\ \ref{eq:g_t5}, Eq.\ \ref{eq:g_t6} to obtain 
\begin{align*}
    -4\mathbb{E}_{q_t} \left \langle \nabla_{(x,m')}\log h,T\nabla_{(x,m')}\log h\right \rangle 
    = -\mathbb{E}_{q_t} \left \langle \nabla_{(x,m')}\log \left ( \frac{q(x,m')}{p(y,x, m')} \right ),T\nabla_{(x,m')}\log \left ( \frac{q(x,m')}{p(y,x, m')} \right ) \right \rangle 
\end{align*}
where
$$
T = \frac{1}{2}\begin{pmatrix}
    a\eta_x I & \left ( \left [ c\eta_x +  a\gamma_x \eta_x \right ]  I + b \mathrm{Hess}_x [\log p_\theta (y,x)] \right )\\
    \left ( \left [ c\eta_x +  a\gamma_x \eta_x \right ]  I + b \mathrm{Hess}_x [\log p_\theta (y,x)] \right ) &   4\gamma_x c\eta_x I + {a}\mathrm{Hess}_x[\log p_\theta (y,x)]
\end{pmatrix}.
$$
In conclusion, we have the following reduction for Eq.\ \ref{}:
\begin{align*}
    &\mathbb{E}_{q_t} \left \langle \nabla_{(x,m')} \left ( \frac{1}{h_\theta(x,m')}  \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')\right ), \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle   \\
= &- 2\gamma_x \mathbb{E}_{q_t} \left \langle \nabla_{x,m'}\nabla_{m'} \log \left ( \frac{q(x,m')}{p(y,x, m')} \right ),
 M\nabla_{x,m'}\nabla_{m'}\log \left ( \frac{q(x,m')}{p(y,x, m')} \right ) \right \rangle_F \\
- &\mathbb{E}_{q_t} \left \langle \nabla_{(x,m')}\log \left ( \frac{q(x,m')}{p(y,x, m')} \right ),T\nabla_{(x,m')}\log \left ( \frac{q(x,m')}{p(y,x, m')} \right ) \right \rangle 
\end{align*}
\textbf{Simplifying Eq.\ \ref{eq:quotient_t2}.} We have
%
\begin{align*}
    &\mathbb{E}_{q_{t}}\left\langle \frac{\nabla_{(x,m')} h_{\theta}(x,m')\left(\nabla_{(x,m')}\right)^{*}\left(M\nabla_{(x,m')} h_{\theta}\right)(x,m')}{h_{\theta}(x,m')^{2}},\begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')}\log h_{\theta}(x,m')\right\rangle 	\\
=&\int p_{\theta}\left(y,dx,dm'\right)\frac{\left(\nabla_{(x,m')}\right)^{*}\left(M\nabla_{(x,m')} h_{\theta}\right)(x,m')}{h_{\theta}(x,m')}\left\langle \nabla_{(x,m')} h_{\theta}(x,m'),\begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} h_{\theta}(x,m')\right\rangle \\
%
	=&\gamma_{x}\int p_{\theta}\left(y,dx,dm'\right)\frac{\left(\nabla_{(x,m')}\right)^{*}\left(M\nabla_{(x,m')} h_{\theta}\right)(x,m')}{h_{\theta}(x,m')}\left\Vert \nabla_{m'}h_{\theta}(x,m')\right\Vert _{2}^{2}.
\end{align*}
Then, using the adjoint of the operator $(\nabla_{(x,m')})^*$ as was described in \ref{sec:lyapunov_fv}. We obtain
\begin{align*}
	=&\gamma_{x}\int p_{\theta}\left(y,dx,dm'\right)\left\langle \nabla_{(x,m')} \left ( \frac{\left\Vert \nabla_{m'} h_{\theta}(x,m')\right\Vert _{2}^{2}}{h_{\theta}(x,m')} \right ),M\nabla_{(x,m')} h_{\theta}(x,m')\right\rangle.
 \end{align*}
 Then, using the quotient rule, we have that 
 \begin{align*}
 %
	=&\gamma_{x}\bar{\mathbb{E}}_\theta \left\langle \frac{\nabla_{(x,m')}\left\Vert \nabla_{m'}h_{\theta}(x,m')\right\Vert _{2}^{2}}{h_{\theta}(x,m')}
    ,M\nabla_{(x,m')} h_{\theta}(x,m')\right\rangle  \\
        &-\gamma_{x}\bar{\mathbb{E}}_\theta\left\langle \frac{\left\Vert \nabla_{m'} h_{\theta}(x,m')\right\Vert^2_2 \nabla_{(x,m')}h_{\theta}(x,m')}{h_{\theta}(x,m')},M\nabla_{(x,m')} h_{\theta}(x,m')\right\rangle  \\
 %
	=2&\gamma_{x}\bar{\mathbb{E}}_\theta\left\langle \frac{\nabla_{(x,m')}\nabla_{m'}h_{\theta}(x,m')\cdot \nabla_{m'} h_{\theta}(x,m')}{h_{\theta}(x,m')},M\nabla_{(x,m')} h_{\theta}(x,m')\right\rangle\\
         &-\gamma_{x}\bar{\mathbb{E}}_\theta\left\langle \frac{\left\Vert \nabla_{m'}h_{\theta}(x,m')\right\Vert^2_2 \nabla_{(x,m')}h_{\theta}(x,m')}{h_{\theta}(x,m')^{2}},M\nabla_{(x,m')} h_{\theta}(x,m')\right\rangle,
 \end{align*}
 where $\cdot$ denotes matrix-vector multiplication. Finally, we write equivalent terms using the Forbenius norm $\langle \cdot, \cdot \rangle_F$. In other words, we have
 %
 \begin{align*}
	=&2\gamma_{x}\bar{\mathbb{E}}_\theta \left\langle \nabla_{(x,m')}\nabla_{m'}h_{\theta}(x,m'),M\frac{\nabla_{(x,m')} h_{\theta}(x,m')}{h_{\theta}(x,m')}\otimes\nabla_{m'} h_{\theta}(x,m')\right\rangle _{F}\\
 %
	-&\gamma_{x}\bar{\mathbb{E}}_\theta \left\langle \frac{\nabla_{(x,m')}h_{\theta}(x,m')}{h_{\theta}(x,m')}\otimes\nabla_{m'}h_{\theta}(x,m'),M\frac{\nabla_{(x,m')}h_{\theta}(x,m')}{h_{\theta}(x,m')}\otimes\nabla_{m'}h_{\theta}(x,m')\right\rangle_F
\end{align*}
%
where $\otimes$ denotes the outer product, and we use the fact that
$$
 \left\Vert \nabla_{m'}h_{\theta}(x,m')\right\Vert \nabla_{(x,m')}h_{\theta}(x,m')=\left(\nabla_{(x,m')}h_{\theta}(x,m')\otimes\nabla_{m'}h_{\theta}(x,m')\right)\cdot \nabla_{m'}h_{\theta}(x,m').
$$
%
\textbf{Simplifying \ref{eq:quotient_t1}.} We will show that 
\begin{align*}
    &\mathbb{E}_{q_t} \left \langle \frac{\nabla_{(x,m')} \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')}{h_\theta(x,m')}, \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle  \\
= &\bar{\mathbb{E}}_\theta \left \langle \nabla_{x,m'}\nabla_{m'}h(x,m'),S\nabla_{x,m'}\nabla_{m'}h(x,m') \right \rangle_F \\
+ & \frac{a\eta_x}{4}\mathbb{E}_\theta [\|\nabla_x h(x,m')\|^2_2 \\
+ &\frac{1}{2} \bar{\mathbb{E}}_\theta \left \langle \nabla_{x} h_\theta (x,m'), \left ( \left [ c\eta_x +  a\gamma_x \eta_x \right ]  I + b \mathrm{Hess}_x [\log p_\theta (y,x)] \right ) \nabla_{m'} h (x,m') \right \rangle \\
+ &\bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} h_\theta (x,m'), \left ( c\eta_x\gamma_x I + \frac{a}{4}\mathrm{Hess}_x[\log p_\theta (y,x)] \right ) \nabla_{m'} h_\theta (x,m')\right \rangle. \\
\end{align*}
We have
%
\begin{align*}
    \mathbb{E}_{q_t} \left \langle \frac{\nabla_{(x,m')} \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')}{h_\theta(x,m')}, \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle  \\
= \bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m'), \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle.
\end{align*}
Since we have
%
\begin{align*}
    \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) &= \left (\nabla_{x} \right )^*  \left( b\nabla_{x} h_\theta + \frac{a}{2} \nabla_{m'} h_\theta  \right ) \\
    &+\left (\nabla_{m'} \right )^* \left( \frac{a}{2}\nabla_{x} h_\theta + c\nabla_{m'} h_\theta  \right ),
\end{align*}
%
we obtain
%
\begin{align}
 &\mathbb{E}_{q_t} \left \langle \frac{\nabla_{(x,m')} \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')}{h_\theta(x,m')}, \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle  \\
= \frac{a}{2} &\bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{x} \right )^* \nabla_{m'} h_\theta + \left (\nabla_{m'} \right )^* \nabla_{x} h_\theta \right ] (x,m'), \begin{pmatrix}0 & -I \\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle \label{eq:nested_t1}\\
&+ b \bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{x} \right )^* \left(\nabla_{x} h_\theta   \right ) \right ] (x,m'), \begin{pmatrix}0 & -I \\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle. \label{eq:nested_t2}\\
&+ c \bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{m'} \right )^* \left(\nabla_{m'} h_\theta \right ) \right ] (x,m'), \begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle. \label{eq:nested_t3}
\end{align}
%
Again, dealing with these three terms individually.

\begin{itemize}
    \item 
    \textbf{Line \ref{eq:nested_t1}.} We have
    %
    \begin{align}
        &\frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{x} \right )^* \nabla_{m'} h_\theta + \left (\nabla_{m'} \right )^* \nabla_{x} h_\theta \right ] (x,m'), \begin{pmatrix}0 & 0 \\
        0 & \gamma_{x}I
        \end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle\\
        + &\frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{x} \right )^* \nabla_{m'} h_\theta + \left (\nabla_{m'} \right )^* \nabla_{x} h_\theta \right ] (x,m'), \begin{pmatrix}0 & -I \\
        I & 0
        \end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle\\
        = \gamma_{x} &\frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} \left [ \left (\nabla_{x} \right )^* \nabla_{m'} h_\theta + \left (\nabla_{m'} \right )^* \nabla_{x} h_\theta \right ] (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle \label{eq:dt_t3}\\
        + &\frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{x} \right )^* \nabla_{m'} h_\theta + \left (\nabla_{m'} \right )^* \nabla_{x} h_\theta \right ] (x,m'), \begin{pmatrix}0 & -I \\
        I & 0
        \end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle \label{eq:dt_t4}
    \end{align}
    We will deal with Equations \ref{eq:dt_t3} and \ref{eq:dt_t4} separately.
    
    \textbf{Line \ref{eq:nested_t1}: Eq. \ref{eq:dt_t3}.} Using the adjoint of $\nabla_{m'}$ and $\nabla_{m'}$, we obtain
    %
    \begin{align*}
        \gamma_{x} &\frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} \left [ \left (\nabla_{x} \right )^* \nabla_{m'} h_\theta + \left (\nabla_{m'} \right )^* \nabla_{x} h_\theta \right ] (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle \\
        =&\gamma_{x} \frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle   \nabla_{m'} h_\theta (x,m'),  \nabla_{x}(\nabla_{m'})^*\nabla_{m'} h_\theta(x,m') \right \rangle \\
    + &\gamma_{x} \frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{x} h_\theta (x,m'), \nabla_{m'}(\nabla_{m'})^* \nabla_{m'} h_\theta(x,m') \right \rangle,
    \end{align*}
    %
    \jl{Fix this gap}
    Since we have that ..., i.e., $\nabla_x$ commutes with $\nabla_{m'}$ and $(\nabla_{m'})^*$
    %
    \begin{align*}
        =&\gamma_{x} \frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle   \nabla_{m'} h_\theta (x,m'),  (\nabla_{m'})^*\nabla_{m'} \nabla_{x} h_\theta(x,m') \right \rangle \\
    + &\gamma_{x} \frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{x} h_\theta (x,m'), \nabla_{m'}(\nabla_{m'})^* \nabla_{m'} h_\theta(x,m') \right \rangle,
    \end{align*}
    %
    We can write this in terms of the commutator of $\nabla_{m'}$ and $(\nabla_{m'})^*$ defined as $[\nabla_{m'}, (\nabla_{m'})^*] v = \nabla_{m'}(\nabla_{m'})^*v - (\nabla_{m'})^*\nabla_{m'}v$.
    %
    Thus, we have 
    %
    \begin{align}
        =&\gamma_{x} {a}\bar{\mathbb{E}}_\theta \left \langle   \nabla_{m'} h_\theta (x,m'),  (\nabla_{m'})^*\nabla_{m'} \nabla_{x} h_\theta(x,m') \right \rangle \\
    + &\gamma_{x} \frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{x} h_\theta (x,m'), [\nabla_{m'}, (\nabla_{m'})^*] \nabla_{m'} h_\theta(x,m') \right \rangle \\
    =&\gamma_{x} {a}\bar{\mathbb{E}}_\theta \left \langle   \nabla_{m'}\nabla_{m'} h_\theta (x,m'),  \nabla_{m'} \nabla_{x} h_\theta(x,m') \right \rangle_F \\
    +&\gamma_{x}\eta_x \frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{x} h_\theta (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle. \label{eq:t2_first}
    \end{align}

    \textbf{Line \ref{eq:nested_t1}: Eq. \ref{eq:dt_t4}.} Expanding the gradient term $\nabla h_\theta = \frac{h_\theta}{2}\left ( \nabla \log q - \nabla \log p_\theta \right ) $, we obtain
    \begin{align*}
        &\bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{x} \right )^* \nabla_{m'} h_\theta + \left (\nabla_{m'} \right )^* \nabla_{x} h_\theta \right ] (x,m'), \begin{pmatrix}0 & -I \\
                    I & 0
        \end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle \\
        =&\frac{1}{2}\bar{\mathbb{E}}_\theta \left ( \left [ \left (\nabla_{x} \right )^* \nabla_{m'} h_\theta + \left (\nabla_{m'} \right )^* \nabla_{x} h_\theta \right ] (x,m')\cdot  (\nabla_{(x,m')})^* \left [
        h_\theta(x,m') \begin{pmatrix}-\nabla_x \log p_\theta (y,x) \\
                    \eta_x m'
        \end{pmatrix} \right ]\right ) \\
        =& \frac{1}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{m', x} h_\theta  (x,m'), \nabla_{x, m'}  \left ( \eta_x m' \cdot  \nabla_x h(x,m')+ \nabla_x \log p_\theta (y,x)\cdot \nabla_{m'}h(x,m') \right ) 
        \right \rangle,
    \end{align*}
    where we have $\cdot$ in the second line for scalar multiplication and $\cdot$ denotes an inner product for the final line.
    To obtain the second line, we use the adjoint operator of $\nabla_{(x,m')}$. It can be seen that the term $\nabla \log q$ does not play any role and can be removed. The final line is obtained by expanding the operator $(\nabla_{(x,m')})^*$ and applying the adjoint of $(\nabla_{(x,m')})^*$.

    In order to simplify the algebra, we define the operator $B[h] = \nabla_x h(x,m')\cdot\eta_x m'  +  \nabla_{m'}h(x,m') \cdot \nabla_x \log p_\theta (y,x)$ where $\cdot$ denotes an inner product or matrix-vector multiplication depending on the type of $h$. The adjoint of $B$ denoted by $B^*$ w.r.t. the inner product $\mathbb{E} \langle \cdot ,\cdot \rangle$ is $B^*= -B$.
    Then we can continue computation with
    \begin{align*}
         &\frac{1}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{m', x} h_\theta  (x,m'), \nabla_{x, m'}  B[h] 
        \right \rangle \\
        &= \frac{1}{2} \left ( \bar{\mathbb{E}}_\theta \left [\left \langle \nabla_{x} h_\theta  (x,m'), \nabla_{m'}  B[h] + \left \langle \nabla_{m'} h_\theta  (x,m'), \nabla_{x}  B[h] 
        \right \rangle
        \right \rangle\right ] \right ) \\
        &= \frac{1}{2} \left ( \bar{\mathbb{E}}_\theta \left [\left \langle \nabla_{x} h_\theta  (x,m'), \nabla_{m'}  B[h] 
        \right \rangle 
        + \left \langle \nabla_{m'} h_\theta  (x,m'), B \nabla_{x}  [h] \right \rangle 
        + \left \langle \nabla_{m'} h_\theta  (x,m'), [\nabla_{x}, B][h] \right \rangle \right ] \right ) \\
        &= \frac{1}{2} \left ( \bar{\mathbb{E}}_\theta \left [\left \langle \nabla_{x} h_\theta  (x,m'), \nabla_{m'}  B[h] 
        \right \rangle 
        - \left \langle B\nabla_{m'} h_\theta  (x,m'), \nabla_{x}  [h] \right \rangle 
        + \left \langle \nabla_{m'} h_\theta  (x,m'), [\nabla_{x}, B][h] \right \rangle \right ] \right ) \\
        &= \frac{1}{2} \left ( \bar{\mathbb{E}}_\theta \left [\left \langle \nabla_{x} h_\theta  (x,m'), [\nabla_{m'},B][h] 
        \right \rangle 
        + \left \langle \nabla_{m'} h_\theta  (x,m'), [\nabla_{x}, B][h] \right \rangle \right ] \right ).
    \end{align*}
    Since we have $[\nabla_{m'}, B][h]=\eta_x \nabla_x h$ and $[\nabla_{x}, B][h]= \mathrm{Hess}[\log p(y,x)]\nabla_{m'}h$, we have
    %
    \begin{align}
        &\frac{1}{2} \left ( \bar{\mathbb{E}}_\theta \left [\left \langle \nabla_{x} h_\theta  (x,m'), [\nabla_{m'},B][h] 
        \right \rangle 
        + \left \langle \nabla_{m'} h_\theta  (x,m'), [\nabla_{x}, B][h] \right \rangle \right ] \right ) \\
        &= \frac{\eta_x}{2}\mathbb{E}_\theta [\|\nabla_x h(x,m')\|^2_2 \\
        &+ \frac{1}{2}\left \langle \nabla_{m'} h_\theta (x,m'), \mathrm{Hess}_x[\log p_\theta (y,x)] \nabla_{m'} h_\theta (x,m')\right \rangle]  \label{eq:t2_last}
    \end{align}
    \textbf{Summary of Line \ref{eq:nested_t1}}. Thus, summing up Line \ref{eq:t2_first} and Line \ref{eq:t2_last}, we have
    \begin{align*}
        \frac{a}{2} &\bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{x} \right )^* \nabla_{m'} h_\theta + \left (\nabla_{m'} \right )^* \nabla_{x} h_\theta \right ] (x,m'), 
        \begin{pmatrix}
            0 & -I \\
            I & \gamma_{x}I
        \end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle \\
    = &\frac{a\eta_x}{4}\mathbb{E}_\theta [\|\nabla_x h(x,m')\|^2_2 
    \\
    + &\frac{a}{4}\left \langle \nabla_{m'} h_\theta (x,m'), \mathrm{Hess}_x[\log p_\theta (y,x)] \nabla_{m'} h_\theta (x,m')\right \rangle \\
    + &\gamma_{x} {a}\bar{\mathbb{E}}_\theta \left \langle   \nabla_{m'}\nabla_{m'} h_\theta (x,m'),  \nabla_{m'} \nabla_{x} h_\theta(x,m') \right \rangle_F\\
    + &\gamma_{x}\eta_x \frac{a}{2}\bar{\mathbb{E}}_\theta \left \langle \nabla_{x} h_\theta (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle.
    \end{align*}

    \item \textbf{Line \ref{eq:nested_t2}}.
    \begin{align*}
     &b \bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{x} \right )^* \left(\nabla_{x} h_\theta   \right ) \right ] (x,m'), \begin{pmatrix}0 & -I \\
    I & \gamma_{x}I
    \end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle \\
    &= b \gamma_x \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} \left [ \left (\nabla_{x} \right )^* \left(\nabla_{x} h_\theta   \right ) \right ] (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle  \\
    &+ b \bar{\mathbb{E}}_\theta \left \langle \left(\nabla_{x} h_\theta   \right ) (x,m'), \nabla_x B [h] (x,m') \right \rangle
    \end{align*}
    %
    Writing this in terms of the commutator, we get 
    %
    \begin{align*}
    &b \bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{x} \right )^* \left(\nabla_{x} h_\theta   \right ) \right ] (x,m'), \begin{pmatrix}0 & -I \\
    I & \gamma_{x}I
    \end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle \\
    &= b \gamma_x \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} \left [ \left (\nabla_{x} \right )^* \left(\nabla_{x} h_\theta   \right ) \right ] (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle \\
    &+ \frac{b}{2} \bar{\mathbb{E}}_\theta \left \langle \nabla_{x} h_\theta (x,m'), [\nabla_x, B] h (x,m') +B\nabla_x h (x,m') \right \rangle \\
    &= b \gamma \bar{\mathbb{E}} \left \langle \nabla_x\nabla_{m'}h(x,m'),\nabla_x\nabla_{m'}h(x,m') \right \rangle_F \\
    &+\frac{b}{2} \bar{\mathbb{E}}_\theta \left \langle \nabla_{x} h_\theta    (x,m'), \mathrm{Hess}_x [\log p_\theta (y,x)] \nabla_{m'} h (x,m') \right \rangle,
    \end{align*}
    %
    where we use the fact that $(\nabla_x)^*$ commutes with $(\nabla_{m'})$.
    \item \textbf{Line \ref{eq:nested_t3}.}
    \begin{align*}
        &c \bar{\mathbb{E}}_\theta \left \langle \nabla_{(x,m')} \left [ \left (\nabla_{m'} \right )^* \left(\nabla_{m'} h_\theta \right ) \right ] (x,m'), \begin{pmatrix}0 & -I\\
        I & \gamma_{x}I
        \end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle \\
        = &c \gamma_{x}\bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} \left [ \nabla_{m'}  \left(\nabla_{m'} h_\theta \right ) \right ] (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle \\
        + &c \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} h_\theta (x,m'), \nabla_{m'} (\nabla_{(x,m')})^* \begin{pmatrix}0 & -I\\
        I & 0
        \end{pmatrix}\nabla_{(x,m')} h_\theta(x,m') \right \rangle \\
        = &c \gamma_{x}\bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} \left [ \left (\nabla_{m'} \right )^* \left(\nabla_{m'} h_\theta \right ) \right ] (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle \\
        + &\frac{c}{2} \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} h_\theta (x,m'), \nabla_{m'} B h_\theta(x,m') \right \rangle.
    \end{align*}
    Writing in terms of the commutator $[\cdot, \cdot]$ and $B$, we have equivalently
    \jl{Need to show the adjoint of $\nabla_{m'}$ w.r.t. the Forbenius norm.}
    %
    \begin{align*}
        c &\gamma_{x}\bar{\mathbb{E}}_\theta \left \langle \left [\left (\nabla_{m'} \right )^* \nabla_{m'} + [\nabla_{m'}, \left (\nabla_{m'} \right )^*] \right ] \nabla_{m'} h_\theta  (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle \\
        +&\frac{c}{2} \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} h_\theta (x,m'), ([\nabla_{m'},B] + B\nabla_{m'}]) h_\theta(x,m') \right \rangle \\
        = &c\gamma  \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} \nabla_{m'} h_\theta  (x,m'), \nabla_{m'}\nabla_{m'} h_\theta(x,m') \right \rangle_F \\
        + &c \gamma_{x}\bar{\mathbb{E}}_\theta \left \langle \left [ \nabla_{m'}, \left (\nabla_{m'} \right )^* \right ] \nabla_{m'} h_\theta  (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle \\
        + &\frac{c}{2} \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} h_\theta (x,m'), B\nabla_{m'} h_\theta(x,m') \right \rangle \\
        + &\frac{c \eta_x}{2}  \bar{\mathbb{E}}_\theta \langle \nabla_x h(x,m'), \nabla_{m'} h(x,m')\rangle.
    \end{align*}
    %
    Using the antisymmetric property of $B$ and that $[\nabla_m, (\nabla_m)^*] v = \eta_x v$, we obtain
    %
    \begin{align*}
        &= c\gamma  \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} \nabla_{m'} h_\theta  (x,m'), \nabla_{m'}\nabla_{m'} h_\theta(x,m') \right \rangle_F \\
        &+c \eta_x \gamma_{x}\bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} h_\theta  (x,m'), \nabla_{m'} h_\theta(x,m') \right \rangle \\
        &+ \frac{c \eta_x}{2}  \bar{\mathbb{E}}_\theta \langle \nabla_x h(x,m'), \nabla_{m'} h(x,m')\rangle.
    \end{align*}
    \item \textbf{Summary of the First term.} Summing up Line \ref{eq:nested_t1}, Line \ref{eq:nested_t2}, and Line \ref{eq:nested_t3}, we obtain
    \begin{align}
         &\mathbb{E}_{q_t} \left \langle \frac{\nabla_{(x,m')} \left (\nabla_{(x,m')} \right )^* \left( M\nabla_{(x,m')} h_\theta  \right ) (x,m')}{h_\theta(x,m')}, \begin{pmatrix}0 & -I\\
            I & \gamma_{x}I
            \end{pmatrix}\nabla_{(x,m')} \log h_\theta(x,m') \right \rangle \\
            &= \gamma_{x} {a}\bar{\mathbb{E}}_\theta \left \langle   \nabla_{m'}\nabla_{m'} h_\theta (x,m'),  \nabla_{m'} \nabla_{x} h_\theta(x,m') \right \rangle_F \label{eq:f_t1}\\
            &+ c\gamma  \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} \nabla_{m'} h_\theta  (x,m'), \nabla_{m'}\nabla_{m'} h_\theta(x,m') \right \rangle_F \label{eq:f_t2}\\
            &+ b \gamma \bar{\mathbb{E}} \left \langle \nabla_x\nabla_{m'}h(x,m'),\nabla_x\nabla_{m'}h(x,m') \right \rangle_F \label{eq:f_t3}\\
            &+ \frac{a\eta_x}{4}\bar{\mathbb{E}}_\theta [\|\nabla_x h(x,m')\|^2_2 \\
            &+ \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} h_\theta (x,m'), \left ( c\eta_x\gamma_x I + \frac{a}{4}\mathrm{Hess}_x[\log p_\theta (y,x)] \right ) \nabla_{m'} h_\theta (x,m')\right \rangle. \\
            &+ \frac{1}{2} \bar{\mathbb{E}}_\theta \left \langle \nabla_{x} h_\theta (x,m'), \left ( \left [ c\eta_x +  a\gamma_x \eta_x \right ]  I + b \mathrm{Hess}_x [\log p_\theta (y,x)] \right ) \nabla_{m'} h (x,m') \right \rangle
    \end{align}
    We can write the sum of \ref{eq:f_t1}, \ref{eq:f_t2}, \ref{eq:f_t3} to obtain
    \begin{align*}
        &{a}\bar{\mathbb{E}}_\theta \left \langle   \nabla_{m'}\nabla_{m'} h_\theta (x,m'),  \nabla_{m'} \nabla_{x} h_\theta(x,m') \right \rangle_F \\
            + &c \bar{\mathbb{E}}_\theta \left \langle \nabla_{m'} \nabla_{m'} h_\theta  (x,m'), \nabla_{m'}\nabla_{m'} h_\theta(x,m') \right \rangle_F\\
            + &b \bar{\mathbb{E}} \left \langle \nabla_x\nabla_{m'}h(x,m'),\nabla_x\nabla_{m'}h(x,m') \right \rangle_F \\
            = &\bar{\mathbb{E}} \left \langle \nabla_{x,m'}\nabla_{m'}h(x,m'),S\nabla_{x,m'}\nabla_{m'}h(x,m') \right \rangle_F
    \end{align*}
\end{itemize}
%
\subsection{Cross terms.} 
\label{sec:xterm}
We will show that
%
\begin{align}
    - &2 \mathbb{E}_{q_t} \left \langle \nabla_{(x,m')}\left \langle \nabla_{(\theta,m)} \log {p_{\theta}(y,x,m')}
, M' \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right \rangle,\begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \delta_{q}F_{\theta_{t}}^{aug}(x,m') \right \rangle \label{eq:xterm_t1} \\
- &2\mathbb{E}_{q}\left[\left\langle \nabla_{(\theta,m)} \nabla_{(x,m')}\left[\delta_{q}F_{\theta_{t}}^{aug}\left(x,m\right)\right]M\nabla_{(x,m')}\left [\delta_{q}F_{\theta_{t}}^{aug}\left(x,m\right) \right ],\begin{pmatrix}0 & -I\\
I & \gamma_{\theta}I
\end{pmatrix}\nabla_{(\theta, m)}
F_{q}^{aug}\left(\theta_{t},m_{t}\right)\right\rangle \right] \label{eq:xterm_t2}\\
&\le L_{g}b
 \left[\left\Vert \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right\Vert ^{2}+\mathbb{E}_{q_t} \left\Vert \nabla_{(x,m')} \delta_{q}F_{\theta_{t}}^{aug}(x,m')\right\Vert ^{2}\right].
\end{align}

We will rewrite the first term, i.e., Eq.\ \ref{eq:xterm_t1} as
\begin{align*}
- 2 \mathbb{E}_{q_t} \left \langle \nabla_{(x,m')}\left \langle \nabla_{(\theta,m)} \log {p_{\theta}(y,x,m')}
, M' \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right \rangle,\begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \delta_{q}F_{\theta_{t}}^{aug}(x,m') \right \rangle \\
 = - 2 \mathbb{E}_{q_t} \left \langle \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right),M' \nabla_{\theta,m}\nabla_{x,m'} \log p(y,x,m')\begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}\nabla_{(x,m')} \delta_{q}F_{\theta_{t}}^{aug}(x,m') \right \rangle,
\end{align*}
and the second term, i.e., Eq.\ \ref{eq:xterm_t2} as
\begin{align*}
    -2\mathbb{E}_{q}\left[\left\langle \nabla_{(\theta,m)} \nabla_{(x,m')}\left[\delta_{q}F_{\theta_{t}}^{aug}\left(x,m\right)\right]M\nabla_{(x,m')}\left [\delta_{q}F_{\theta_{t}}^{aug}\left(x,m\right) \right ],\begin{pmatrix}0 & -I\\
I & \gamma_{\theta}I
\end{pmatrix}\nabla_{(\theta, m)}
F_{q}^{aug}\left(\theta_{t},m_{t}\right)\right\rangle \right] \\
=-2\mathbb{E}_{q}\left[\left\langle \begin{pmatrix}0 & -I\\
I & \gamma_{\theta}I
\end{pmatrix}^\top \nabla_{(\theta,m)} \nabla_{(x,m')}\left[\delta_{q}F_{\theta_{t}}^{aug}\left(x,m\right)\right]M\nabla_{(x,m')}\left [\delta_{q}F_{\theta_{t}}^{aug}\left(x,m\right) \right ],\nabla_{(\theta, m)}
F_{q}^{aug}\left(\theta_{t},m_{t}\right)\right\rangle \right].
\end{align*}
Hence the sum of Eq.\ \ref{eq:xterm_t1} and Eq.\ \ref{eq:xterm_t2} is given by
$$
-2\mathbb{E}_{q}\left[\left\langle A(x,m) \nabla_{(x,m')}\left [\delta_{q}F_{\theta_{t}}^{aug}\left(x,m\right) \right ],\nabla_{(\theta, m)}
F_{q}^{aug}\left(\theta_{t},m_{t}\right)\right\rangle \right].
$$
and so we focus on the matrix 
\begin{align*}
A:= \begin{pmatrix}0 & -I\\
I & \gamma_{\theta}I
\end{pmatrix}^\top \nabla_{(\theta,m)} \nabla_{(x,m')}\left[\delta_{q}F_{\theta_{t}}^{aug}\left(x,m\right)\right]M 
+ 
    M' \nabla_{\theta,m}\nabla_{x,m'} \log p(y,x,m')\begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix}.
\end{align*}
Using the fact that $\nabla_{\theta,m}\nabla_{x,m'}\delta_{q}F_{\theta_{t}}\left(x,m'\right)=\nabla_{\theta,m}\nabla_{x,m'}\log\frac{q\left(x,m'\right)}{p_{\theta}\left(x,y,m'\right)}=-\nabla_{\theta,m}\nabla_{x,m'}\log p_{\theta}\left(x,y,m'\right)$, we obtain
\begin{align*}
- &\begin{pmatrix}0 & -I\\
I & \gamma_{\theta}I
\end{pmatrix}^\top \nabla_{(\theta,m)} \nabla_{(x,m')}\log p_{\theta}\left(x,y,m'\right)M 
+ 
    M' \nabla_{\theta,m}\nabla_{x,m'} \log p(y,x,m')\begin{pmatrix}0 & -I\\
I & \gamma_{x}I
\end{pmatrix} \\
&= \begin{pmatrix}0 & -b\nabla_{\theta}\nabla_{x}\log p\left(x,y\right)\\
b\nabla_{\theta}\nabla_{x}\log p\left(x,y\right) & 0
\end{pmatrix}.
\end{align*}
Hence, we have
\begin{align}
    - \mathbb{E}_{q_t}\left \langle \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right),\begin{pmatrix}0 & -b\nabla_{\theta}\nabla_{x}\log p\left(x,y\right)\\
b\nabla_{\theta}\nabla_{x}\log p\left(x,y\right) & 0
\end{pmatrix}\nabla_{(x,m')} \delta_{q}F_{\theta_{t}}^{aug}(x,m') \right \rangle \nonumber \\
=
b \mathbb{E}_{q_t}\left \langle \nabla_{\theta} F_{q}^{aug}\left(\theta,m\right),
\nabla_{\theta}\nabla_{x}\log p\left(x,y\right)
\nabla_{m'} \delta_{q}F_{\theta_{t}}^{aug}(x,m') \right \rangle 
\label{eq:xterm_sim_t1}\\ 
-
b\mathbb{E}_{q_t}\left \langle \nabla_{m} F_{q}^{aug}\left(\theta,m\right),
\nabla_{\theta}\nabla_{x}\log p\left(x,y\right)
\nabla_{x} \delta_{q}F_{\theta_{t}}^{aug}(x,m') \right \rangle \label{eq:xterm_sim_t2}
\end{align}
%
Under our Lipschitz gradient assumption and concave potential $U_\theta(y, x)$ w.r.t. $\theta$ and $x$, we have the following relationship
$$
 0 \le z^\top \nabla_{\theta, x} \nabla_{\theta, x} U(y, x) z \le L_g \|z \|^2, \forall z \in \mathbb{R}^{d_\theta + d_x}.
$$
Hence, we have the following lower bound
\begin{align*}
     \theta^\top \nabla_{\theta} \nabla_{x} U(y, x) v  &\ge  - \frac{1}{2}\left (\theta^\top \nabla_\theta \nabla_\theta U_\theta (y,x) \theta  + v^\top \nabla_x  \nabla_x U(y,x)v  \right )  \\
     &\ge - \frac{L_g}{2} \|z\|^2,
\end{align*}
for all $ z:= \begin{bmatrix}
    \theta \\
    v
\end{bmatrix} \in \mathbb{R}^{d_\theta + d_x}$. Similarly, an upper bound is given by
\begin{align*}
    {\theta^\top} \nabla_{\theta} \nabla_{x}U(y, x) v  &\le \frac{L_g}{2} \left ( \|\theta \|^2+\|v\|^2\right ) - \frac{1}{2}\left (\theta^\top \nabla_\theta \nabla_\theta U_\theta (y,x) \theta  + v^\top \nabla_x  \nabla_x U(y,x)v  \right ) \\
&\le \frac{L_g}{2} \left ( \|\theta \|^2+\|v\|^2\right ),
\end{align*}
for all $ z:= \begin{bmatrix}
    \theta \\
    v
\end{bmatrix} \in \mathbb{R}^{d_\theta + d_x}$. Using the above upper, we can upper bound Eq.\ \ref{eq:xterm_sim_t2}
\begin{align*}
     b\mathbb{E}_{q_t}\left \langle \nabla_{m} F_{q}^{aug}\left(\theta,m\right),
\nabla_{\theta}\nabla_{x}U_\theta \left(x,y\right)
\nabla_{x} \delta_{q}F_{\theta_{t}}^{aug}(x,m') \right \rangle \\
\le \frac{L_{g}b}{2} \mathbb{E}_{q_t}
\left[\left\Vert \nabla_{m} F_{q}^{aug}\left(\theta,m\right)\right\Vert ^{2}+\left\Vert \nabla_{x} \delta_{q}F_{\theta_{t}}^{aug}(x,m') \right\Vert ^{2}\right].
\end{align*}
As for Eq.\ \ref{eq:xterm_sim_t1}, we upper bound it with the lower bound 
\begin{align*}
    - b \mathbb{E}_{q_t}\left \langle \nabla_{\theta} F_{q}^{aug}\left(\theta,m\right),
\nabla_{\theta}\nabla_{x}U_\theta \left(x,y\right)
\nabla_{m'} \delta_{q}F_{\theta_{t}}^{aug}(x,m') \right \rangle \\
\le \frac{L_{g}b}{2}
 \mathbb{E}_{q_t} \left[\left\Vert \nabla_{\theta} F_{q}^{aug}\left(\theta,m\right)\right\Vert ^{2}+\left\Vert \nabla_{m'} \delta_{q}F_{\theta_{t}}^{aug}(x,m')\right\Vert ^{2}\right].
\end{align*}
So we have
\begin{align*}
      - &\mathbb{E}_{q_t}\left \langle \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right),\begin{pmatrix}0 & -b\nabla_{\theta}\nabla_{x}\log p\left(x,y\right)\\
b\nabla_{\theta}\nabla_{x}\log p\left(x,y\right) & 0
\end{pmatrix}\nabla_{(x,m')} \delta_{q}F_{\theta_{t}}^{aug}(x,m') \right \rangle 
\\
\le &\frac{L_{g}b}{2}
 \left[\left\Vert \nabla_{(\theta,m)} F_{q}^{aug}\left(\theta,m\right)\right\Vert ^{2}+\mathbb{E}_{q_t} \left\Vert \nabla_{(x,m')} \delta_{q}F_{\theta_{t}}^{aug}(x,m')\right\Vert ^{2}\right].
\end{align*}
\jl{Is this how?}
\adam{Look plausible\dots}

==> unused/juanstuff.tex <==
I'm gonna use the notation of ParEM Appendix A. Note that if we treat $\cal{M}:=\Theta\times\cal{P}(\cal{X})$ as a manifold, we can also treat $\frak{M}:=\cal{M}\times \cal{T}\cal{M}$ as a manifold with:
%
\begin{itemize}
	\item tangent spaces $(\cal{T}\frak{M}:=\cal{T}\cal{M}\times \cal{T}\cal{M})_{z\in\frak{M}}$,
	\item cotangent spaces $(\cal{T}^*\frak{M}:=\cal{T}^*\cal{M}\times \cal{T}^*\cal{M})_{z\in\frak{M}}$,
	\item and duality pairing 
	$$\iprod{(\zeta_1,\zeta_2)}{(\xi_1,\xi_2)}=\iprod{\zeta_1}{\xi_1}+\iprod{\zeta_2}{\xi_2}\quad\forall (\zeta_1,\zeta_2)\in\cal{T}\frak{M},\enskip (\xi_1,\xi_2)\in\cal{T}^*\frak{M}.$$
\end{itemize}

\section{Euler-Langrange equations and Hamiltonian flows for Riemannian manifolds}

Wibisono and friends derived accelerated gradient descent by discretizing an Euler-Lagrange equation. We follow a similar approach here starting from the following Euler-Lagrange equation:
%
\begin{equation}\label{eq:el}\frac{d}{dt}\left[\delta L_{(\tau,\rho)}((\theta_t, q_t), (\dot{\theta}_t, \dot{q}_t))\right]=\delta L_{(\theta, q)}((\theta_t, q_t), (\dot{\theta}_t, \dot{q}_t))\quad\forall t\geq0,\end{equation}
%
where $(\theta_t, q_t)_{t\geq0}$ denotes a differentiable curve in $\cal{M}$,  $L$ is the functional on $\frak{M}$ defined by
%
$$L((\theta, q), (\tau,\rho)):= \frac{1}{2}g_{(\theta,q)}((\tau,\rho), (\tau,\rho))-\cal{F}(\theta,q)\quad\forall (\theta, q)\in\cal{M},\enskip (\tau,\rho)\in\cal{T}\cal{M},$$
%
and $\delta L = (\delta L_{(\theta,q)},\delta L_{(\tau,\rho)})$  denotes $L$'s first variation. 

\begin{example}Suppose that, as in the other paper,
	%
	$$g_{(\theta,q)}((\tau, \rho),(\tau',\rho'))=\iprod{\tau}{\tau'}_2+\sf{g}_q(\rho,\rho'),$$
	%
	where $\iprod{\cdot}{\cdot}_2$ denotes the Euclidean inner product and $\sf{g}_q$ the Wasserstein 2 metric. But, 
	%
	\begin{align*}\delta_\tau [\tau\mapsto \iprod{\tau}{\tau'}_2] &= 2\tau\\
		\delta_q[q\mapsto \sf{g}_q(\rho,\rho)] &= -\norm{\nabla_x \frac{C}{10}}^2\quad\text{where $\frac{C}{10}$ satisfies}\quad\rho= \sf{G}_q^{-1}\frac{C}{10}=-\nabla_x\cdot (q\nabla_x \frac{C}{10}),\\
		\delta_\rho[\rho\mapsto \sf{g}_q(\rho,\rho)]&=2\sf{G}_q\rho.
	\end{align*}
	(The last are according to Wuchen and buds in the proof of Theorem 1 in `WASSERSTEIN HAMILTONIAN FLOWS'). Hence,
	%
	\begin{align}
		\delta_\theta L(\theta,q) &= -\delta_\theta\cal{F}(\theta,q),\label{eq:elp1} \\ %= \int \nabla_\theta \ell(\theta,x)q(x)dx
		\delta_q L(\theta,q,\rho) &=\frac{1}{2}\delta_q [q\mapsto\sf{g}_q(\rho,\rho)]-\delta_q\cal{F}(\theta,q)=-\frac{1}{2}\norm{\nabla_x \frac{C}{10}}^2-\delta_q\cal{F}(\theta,q),\\
		\delta_\tau L(\tau) &=\tau,\nonumber\\
		\delta_\rho L(q,\rho) &=\frac{1}{2}\delta_\rho[\rho\mapsto \sf{g}_q(\rho,\rho)]=\sf{G}_q\rho=\frac{C}{10}.\nonumber
	\end{align}
	%
	where $\frac{C}{10}=\sf{G}_q\rho$ satisfies $\rho=-\nabla_x\cdot (q\nabla_x \frac{C}{10})$. Using the last two equations,
	%
	\begin{align}
		\frac{d}{dt}[\delta_\tau L(\dot{\theta}_t)]=\ddot{\theta}_t,\quad 
		\frac{d}{dt}[\delta_\rho L(q_t,\dot{q}_t)]=\frac{d}{dt}[\sf{G}_{q_t}\dot{q}_t]=\sf{G}_{q_t}\ddot{q}_t+\sf{G}_{q_t}\left[\nabla_x\cdot (\dot{q}_t \nabla_x [\sf{G}_{q_t}\dot{q}_t])\right].\label{eq:elp2}
	\end{align}
	%
	where the last equality was shown in Wuchen's proof.
\end{example}

\textbf{The primal forumaltion:} We break \eqref{eq:el} into
%
\begin{align*}
	\frac{d}{dt}[\delta_\tau L(\dot{\theta}_t)]=\delta_\theta L(\theta_t,q_t),\quad 
	\frac{d}{dt}[\delta_\rho L(q_t,\dot{q}_t)]=\delta_q L(\theta_t,q_t,\rho_t).
\end{align*}
%
Plugging (\eqref{eq:elp1}--\eqref{eq:elp2}) into the above, we obtain
%
\begin{align}
	\ddot{\theta}_t&=-\delta_\theta\cal{F}(\theta_t,q_t)=-\nabla_\theta\cal{F}(\theta_t,q_t),\\
	\sf{G}_{q_t}\ddot{q}_t+\sf{G}_{q_t}\left[\nabla_x\cdot (\dot{q}_t \nabla_x \frac{C}{10}_t)\right]&=-\frac{1}{2}\norm{\nabla_x \frac{C}{10}_t}^2-\delta_q\cal{F}(\theta_t,q_t),\nonumber
	%\frac{\log(p_{\theta_t}(\cdot,y))}{q_t}
\end{align}
%
where $\frac{C}{10}_t=G_{q_t}\dot{q}_t$ satisfies $\dot{q}_t=-\nabla_x\cdot (q_t\nabla_x \frac{C}{10}_t)$. Multiplying the second equation through by $G_{q_t}^{-1}$, we find that
%
\begin{equation}
	\ddot{q}_t+\left[\nabla_x\cdot ([\dot{q}_t+q_t\nabla^2_x \frac{C}{10}_t] \nabla_x \frac{C}{10}_t)\right] =-\nabla_q\cal{F}(\theta_t,q_t).\label{eq:primalform}
\end{equation}
%
Note the LHS is the analogue of the covariant derivative of $\dot{q}_t$ along $q_t$ (see below for more on this) and the middle two terms add up to the analogue of the Christofell symbols (See Section 2 of Wuchen's thing).

\textbf{The dual formulation and the SDEs:}We can also re-write the above in `dual coordinates' as:
%
\begin{align}
	\dot{\theta}_t&=\varphi_t,\quad
	\dot{q}_t=-\nabla_x\cdot (q_t\nabla_x \frac{C}{10}_t),\quad
	\dot{\varphi}_t=-\delta_\theta\cal{F}(\theta_t,q_t),\quad
	\dot{\frac{C}{10}}_t=-\frac{1}{2}\norm{\nabla_x \frac{C}{10}_t}^2-\delta_q\cal{F}(\theta_t,q_t).\label{eq:dualform}
\end{align}
%
Now, suppose that $(\theta_t,q_t,\varphi_t,\frac{C}{10}_t)_{t\geq0}$ solve the above. By definition, the law of the solution of
%
$$\dot{x}_t=m_t,\quad x_0\sim q_0,$$
%
with $m_t:=\nabla_x\frac{C}{10}_t(x_t)$, 
satisfies the same IVP as $(q_t)_{t\geq0}$ and, hence, equals $(q_t)_{t\geq0}$. Moreover,
%
\begin{align*}\dot{m}_t=\frac{d}{dt}\nabla_x\frac{C}{10}_t(x_t)&=\nabla_x^2\frac{C}{10}(x_t)\dot{x}_t+\nabla_x \dot{\frac{C}{10}}_t(x_t)\\
	&=\nabla_x^2\frac{C}{10}(x_t)\nabla_x\frac{C}{10}_t(x_t)-\nabla_x\left[\frac{1}{2}\norm{\nabla_x \frac{C}{10}_t(x_t)}^2+\delta_q\cal{F}(\theta_t,q_t)(x_t)\right]\\
	&=-\nabla_q\cal{F}(\theta_t,q_t)(x_t),\quad m_0=\nabla_x\frac{C}{10}_0(x_0).
\end{align*}
%
%
The law of the above two ODEs coincides with that of 
%
\begin{align*}
	dX_t=M_tdt,\quad dM_t=-\ell(\theta_t,X_t)dt+\sqrt{2}dW_t,\quad M_0=\nabla \frac{C}{10}_0(X_0), X_0\sim q_0.
\end{align*}
\jl{ I think there is something off here. The above SDE satisfies
	$$
	\partial_t p_t (x,m) = - \nabla \cdot (p_t(x,m) \begin{bmatrix}
		m_t \\
		-\ell(\theta_t,X_t) - \nabla_m \log p_t(x,m)
	\end{bmatrix})
	$$
	Rather than the
	$$
	\partial_t p_t (x,m) = - \nabla \cdot (p_t(x,m) \begin{bmatrix}
		m_t \\
		-\ell(\theta_t,X_t) - \nabla_x \log p_t(x)
	\end{bmatrix})
	$$
	As suggested in $\dot{m}_t$ calculations. Am I misunderstanding something here?
}
\juanl{You're not, I'm the one who messed up. They're not the same thing: this is discussed in Appendix~III of Taghvaei 2019.}
%
Putting the above together with the equations for $(\theta_t,\varphi_t)$ we get the SDEs we're interested in.

==> unused/lsi.tex <==
\section{On (Extended) Log Sobolev Inequality}

% \begin{equation*}
%      I(\theta_t, q_t) := - \frac{\rm{d}}{\rm{d}t}\cal{E}(\theta_t, q_t)
% \end{equation*}
% From \citet[page 21]{Kuntz2022}, under $\lambda$-strongly concave? assumptions on $\ell$, we have
% \begin{equation*}
%      \frac{\rm{d}}{\rm{d}t} I(\theta_t, q_t) \le 2 \lambda I(\theta_t, q_t) \implies I(\theta_t, q_t) \le I(\theta_0, q_0) \exp(- 2\lambda t)
% \end{equation*}
% Then, we have
% \begin{equation*}
%     \cal{E}(\theta_0, q_0) - \cal{E}(\theta_t, q_t)  = \int_0^t  I(\theta_t, q_t)\rm{d}t \le I(\theta_0, q_0) \frac{(1- \exp(-2\lambda t))}{2\lambda}.
% \end{equation*}
% Hence, if $\lim_{t\rightarrow \infty} \cal{E} (\theta_t, q_t) = \cal{E}(\theta^*, p_{\theta^*}(\cdot|y)) = - \log p_{\theta^*}(y)$, we have that $\cal{E}$ satisfies the extended log-Sobolev inequality assumption \cref{ass:logsobolev}, i.e., 
% $$
% \cal{E}(\theta_0, q_0) +\log p_{\theta^*} (y) 
% \le I(\theta_0, q_0) \frac{(1- \exp(-2\lambda t))}{2\lambda}.
% $$

% $$
% d\theta_t
% $$
\begin{definition}[Log Sobolev Inequality]
	
\end{definition}
\begin{definition}[Strong Convexity]
	
\end{definition}
\begin{proposition}
    If for all $x$, the map $\theta \mapsto \ell(\theta, x)$ is strongly concave, i.e., for all $x$, we have
    $$
    \ell (\theta, x) \ge \ell (\theta', x) + \iprod{\nabla_\theta\ell (\theta', x) }{\theta - \theta'} + \frac{\mu}{2} \|\theta - \theta'\|^2,\quad \forall \theta, \theta',
    $$
    then $\theta \mapsto \cal{E}(\theta, q)$ is strongly-concave.
\end{proposition}
\begin{proof} Simply, we have
    $$
    \cal{E}(\theta, q) = \int \ell(\theta, x) q(\rm{d}x) \ge \cal{E}(\theta', q) + \iprod{\nabla_\theta \cal{E}(\theta', q)}{\theta - \theta'}+ \frac{\mu}{2} \|\theta - \theta'\|^2.
    $$
\end{proof}
\begin{proposition}
    Assume that
    \begin{enumerate}
        \item $\theta^*$ is a unique maximizer of the marginal likelihood,
        \item for all $\theta$, the posterior $p_{\theta}(x|y)$ satisfies the log-sobolev inequality,
        \item the map $\theta \mapsto \ell (\theta, x)$ is strongly concave for all $x$,
    \end{enumerate} 
    Then, $\cal{E}$ satisfies the extended Log Sobolev inequality.
\end{proposition}
\begin{proof}
    Recall that 
    $$
    \left\Vert \nabla{\cal E}\left(\theta,q\right)\right\Vert ^{2}=\left\Vert \nabla_{\theta}{\cal E}\left(\theta,q\right)\right\Vert ^{2}+\left\Vert \nabla_{x}\log\frac{q}{p_{\theta}}\right\Vert _{q}^{2}
    $$
    From the log Sobolev assumption (2), we have
    $$
    \left\Vert \nabla_{x}\log\frac{q}{p_{\theta}}\right\Vert _{q}^{2} = \left\Vert \nabla_{x}\log\frac{q}{p_{\theta}(\cdot|y)}\right\Vert _{q}^{2} \ge \frac{1}{C_{LS}}\sf{KL}(q|p_{\theta}(\cdot|y)) = \frac{1}{C_{LS}} (\cal{E}(\theta, q) + \log p_\theta(y)).
    $$
    Under assumption (3), we will show that
    $$
    C\left\Vert \nabla_{\theta}{\cal E}\left(\theta,q\right)\right\Vert ^{2} \ge {\cal E}\left(\theta,q\right)-{\cal E}\left(\theta^{*},q\right).
    $$
    From \Cref{prop}, we have that $\theta \mapsto \cal{E}(\theta, q)$ is strongly-concave. Then we have
    $$
    \min_\theta  \cal{E}(\theta, q) \ge \min_\theta  \left \{\cal{E}(\theta', q) + \iprod{\nabla_\theta \cal{E}(\theta', q)}{\theta - \theta'}+ \frac{\mu}{2} \|\theta - \theta'\|^2 \right \}.
    $$
    The optimum is achieved  with $\theta = \theta ' - \frac{1}{\mu} \nabla_\theta \cal{E}(\theta', q)$. Hence we have the inequality:
    $$
    \cal{E}(\theta^*, q)\ge \min_\theta  \cal{E}(\theta, q) \ge \cal{E}(\theta', q)- \frac{1}{2\mu}\|\nabla_\theta \cal{E}(\theta', q)\|^2.
    $$
    Hence we have 
    $$
    \frac{1}{2\mu}\|\nabla_\theta \cal{E}(\theta, q)\|^2 \ge \cal{E}(\theta, q) - \cal{E}(\theta^*, q) \
    $$
    Recall that since
    $
     \cal{E}(\theta, q)= - \log p_\theta(y) + \sf{KL}(q, p_\theta(\cdot|y)) \ge - \log p_\theta(y),
    $
    we obtain
    $$
     \frac{1}{2\mu}\|\nabla_\theta \cal{E}(\theta, q)\|^2 \ge - \log p_\theta(y)+ \log p_{\theta^*}(y) + \sf{KL}(q, p_{\theta}(\cdot|y)) -\sf{KL}(q, p_{\theta *}(\cdot|y)). 
    $$
    To conclude, combining 
    $$
     \left\Vert \nabla_{x}\log\frac{q}{p_{\theta}}\right\Vert _{q}^{2} + \|\nabla_\theta \cal{E}(\theta, q)\|^2 \ge \frac{1}{C} ( \cal{E}(\theta, q) - 
    $$
    where $C= \max \{\}$ 
\end{proof}

==> unused/old.tex <==

% We are concerned with the training of (probabilistic) latent variable  models of the form $p_\theta (y, x)$ where $y \in \mathbb{R}^{d_y}$ denotes an observed variable, $x \in \mathbb{R}^{d_x}$ an unobserved (or \emph{latent}) one, and $\theta$ the model parameters. Ideally, we choose $\theta$ by maximizing the marginal likelihood $p_\theta (y) := \int p_\theta (y, x)dx$. However, the marginal likelihood is typically intractable; thus, direct optimization is impossible.

% One way of circumventing this intractability is by constructing a tractable objective on an extended space. Working instead on the space of parameters $\bb{R}^{d_\theta}$ and probability distributions over the latent space $\mathbb{R}^{d_x}$, we minimize the free energy functional $\cal{E}: \mathbb{R}^{d_\theta} \times \mathcal{P(\mathbb{R}}^{d_x})$ which is defined as
% %
% $$
% \mathcal{E}(\theta, q) := \int \log \left ( \frac{q(x)}{p_\theta(y,x)}\right ) q(dx),
% $$
% %
% where $\mathcal{P(\mathbb{R}}^{d_x})$ is space of probability distributions on $\mathbb{R}^{d_x}$\footnote{We assume that $q \in \mathcal{P(\mathbb{R}}^d)$ admit a density w.r.t.\ to the Lebesgue measure and has finite second moments.}. The free energy is related to the log marginal likelihood through the following relationship:
% %
% \begin{align*}
%     \log p_\theta (y) &= - \cal{E}(\theta, q)  + \mathrm{KL}(q(x) \| p_\theta(x|y)) \ge - \cal{E}(\theta, q).
% \end{align*}
% %
% Hence, minimizing $\cal{E}$ is equivalent to maximizing a lower bound on the log marginal likelihood.

% Various methods for training latent variable has been proposed that minimize the free energy, such as expectation maximization which use coordinate ascent approach \citep{neal1998view}. Recently, \citet{Kuntz2022} proposed several particle-based algorithms emulating the gradient descent algorithm (GD): a popular first-order method for minimizing a function over Euclidean space. GD entails taking small steps in the negative gradient direction, which specifies the direction of steepest descent. However, GD does not achieve optimal oracle rates \citep{nemirovskij1983problem}. 

% \citet{nesterov1983method} found that incorporating momentum into gradient descent produced accelerated algorithms that were faster and achieved optimal rates. In the context of machine learning, \citet{sutskever2013importance} demonstrated that using momentum can eliminate the performance gap between (stochastic) gradient descent and a second-order optimization method known as Hessian-Free optimization \citep{martens2010deep}. \citet{sutskever2013importance} attributed this to the ``transient'' phase of training neural networks being more important than local convergence. In the transient phase, the direction of greatest descent persists through gradient updates which momentum-based methods can abuse.

% Given the success of momentum, in this work, we ask if we can accelerate the particle methods of \citet{Kuntz2022} by introducing momentum to optimize over the product space $\mathbb{R}^{d_\theta} \times \mathcal{P(\mathbb{R}}^{d_x})$.

% \newpage

% In this section, we i) review the construction of the algorithm from \citet{Kuntz2022}, ii) review gradient methods for optimisation on $\mathbb{R}^{d}$ which achieve accelerated convergence rates, and some relevant interpretations stemming from dynamical systems, and iii) describe how these interpretations may be extended to problems of optimisation over $\mathcal{P}\left(\mathbb{R}^{d}\right)$. This will lay the groundwork for our later developments in optimisation over $\mathbb{R}^{d_{\theta}}\times\mathcal{P}\left(\mathbb{R}^{d_{x}}\right)$. 

% \subsection{Particle-based Maximum Likelihood.}

% We first review the particle EM methods of \citet{Kuntz2022}. While the authors developed a number of distinct algorithms, we focus here on a particular instance, the `particle gradient descent' (PGD) algorithm. PGD is derived by considering a gradient flow of the free energy functional $\mathcal{E}$ over the joint space of $\left(\theta,q\right)$ with respect to the Wasserstein-2 geometry \citep{jordan1998variational}. Other geometries can also be used, and will lead to different dynamics and algorithms; see e.g. \cite{duncan2019geometry,sharrock2023coinem} for examples. 

% Given an initial point $\left(\theta_{0},q_{0}\right)$, the gradient flow in question then evolves according to the dynamics
% %
% \begin{align*}
%     \dot{\theta}_{t}	&=-\nabla_{\theta}\mathcal{E}\left(\theta_{t},q_{t}\right) \\
%     \dot{q}_{t}	&=-\nabla_{W}\mathcal{E}\left(\theta_{t},q_{t}\right),
% \end{align*}
% %
% where $\nabla_{\theta}$ denotes the standard Euclidean gradient in $\mathbb{R}^{d_{\theta}}$ and $\nabla_{W}$ denotes the `Wasserstein gradient' of $\mathcal{E}$ with respect to the distribution $q$. Deferring technical details to the Appendix, with $\mathcal{E}$ as our particular free energy functional, one computes that 
% %
% \begin{align*}
%     \nabla_{\theta}\mathcal{E}\left(\theta,q\right)	&=\int q\left(\mathrm{d}x\right) \cdot \nabla_{\theta}\ell\left(\theta,x\right) \\
%     \nabla_{W}\mathcal{E}\left(\theta,q\right)	&=-\nabla_{x}\cdot\left(q\cdot\nabla_{x}\left(\ell\left(\theta,x\right)-\log q\left(x\right)\right)\right),
% \end{align*}
% %
% where $\ell \left( \theta, x \right) = \log p_\theta \left( y, x \right)$ and $\nabla_{x}\cdot$ denotes the divergence operator which sends vector fields to scalar fields.

% % \citet{Kuntz2022} proposed several algorithms utilizing various optimization algorithms to optimize $\cal{E}$. One of which is a discretization of the gradient flow of $\cal{E}$ resulting in a (particle) gradient descent algorithm which we call $\texttt{PGD}$.

% % Given some initial point $(\theta_0, q_0)$, the gradient flow of $\cal{E}$ is described by
% % $$
% % \dot{\theta}_t = - \nabla_\theta \cal{E}(\theta_t, q_t), \quad \dot{q}_t = - \nabla_W \cal{E}(\theta_t, q_t),
% % $$
% % where the gradient $\nabla_\theta$ is taken in the usual Euclidean sense and the gradient $\nabla_W$ is interpreted in the Wasserstein-2 sense \citep{jordan1998variational}. We have
% % %
% % $$
% %  \nabla_\theta \cal{E}(\theta_t, q_t) = - \int \nabla_\theta \ell (\theta, x)q_t(dx) , \quad \nabla_W \cal{E}
% % (\theta, q):= - \nabla_x \cdot (q \nabla_x {\delta_q \cal{E}[\theta, q]}),
% % $$
% % %
% % where $\ell(\theta, x):= \log p_\theta(y, x)$, $\delta_q \cal{E}[\theta , q]= \log {q}/{p_\theta (y, \cdot )} : \mathbb{R}^{d_x} \rightarrow \mathbb{R}$ denotes the first variation of $\cal{E}$ \citep[Lemma 1]{Kuntz2022}, and $\nabla \cdot$ is the divergence operator. One can use different geometries that will give rise to different algorithms. For instance, endowing the space $\cal{P}(\mathbb{R}^{d_x})$ with Stein geometry \citep{duncan2019geometry} gives rise to Stein Variational Gradient Descent Expectation Maximization \citep{sharrock2023coinem}.

% % In order to deal with the intractabilities that arises from the gradients $(\nabla_\theta, \nabla_W)$, \citet{Kuntz2022} exploit the fact that $\nabla_W \cal{E}$ describes a transport equation, and obtains the gradient flow of $\cal{E}$ as the following McKean-Vlasov SDE:
% % %
% % \begin{align}
% % 	d\theta_t &= \int \nabla_\theta \ell (\theta_t, x)q_t(dx) dt, \\
% % 	q_t = \mathrm{Law}(X_t): dX_t &= \nabla_x  \ell (\theta_t, X_t)dt + \sqrt{2}dW_t \label{eq:pgd_flow}.
% % \end{align}
% % %
% % where $W_t$ is standard Wiener process. Taking the $M$-particle approximation of $q_t$, i.e., $q_t \approx \frac{1}{M} \sum_{i=1}^M \delta_{X^i_t}$, with each $X_t^i$ a (conditionally upon $\theta$ independent) copy of $X_t$, we arrive at the following approximate gradient flow by approximating the integral with particles:
% % \begin{align}
% %     d\theta_t &= \left [\frac{1}{M} \sum_{i=1}^M \nabla_\theta \ell (\theta_t, X_t^i) \right ] dt, \\
% %     \forall i \in [M]:  dX^i_t &= \nabla_x  \ell (\theta_t, X^i_t)dt + \sqrt{2}dW^i_t,\  \label{eq:pgd}
% % \end{align}
% % where $[M] := \{1,...,M\}$ and $\{W_t^i\}_{i=1}^M$ denotes a collection of $M$ independent Wiener processes.
% % Utilizing Euler-Maruyama discretization scheme with a step-size $h>0$ yields \texttt{PGD}'s recursion:
% % %
% % \begin{align*}
% %     \theta_{k+1} &= \theta_k + \frac{h}{M} \sum_{i=1}^M \nabla_\theta \ell ({\theta_k}, X^i_k), \\
% %     \forall i \in [M]: X_{k+1}^i &=  X^i_k + h\nabla_x\ell({\theta_k}, X^i_k) + \sqrt{2h}\epsilon^i_k .
% % \end{align*}
% % where $\epsilon^i_k \overset{\textrm{i.i.d.}}{\sim} \mathcal{N}(0_{d_x}, I_{d_x})$, for some initialization $(\theta_0, \{X_0^i\}_{i=1}^M)$.

% \adaml{With the current structure there's something of an abrupt transition here.}

% \subsection{Accelerating Gradient Descent in $\mathbb{R}^d$.}
% \label{sec:euclidean_momentum}

% Consider now the task of minimising a function $f:\mathbb{R}^{d}\to\mathbb{R}$. In machine learning, it is commonplace to approach such tasks by use of first-order optimisation methods, such as gradient descent. Despite its simplicity and widespread use, it is by now well-understood that under various circumstances, there exist methods with appreciably faster convergence than gradient descent; see e.g. \cite{nemirovskij1983problem}. While there are various proposed explanations for this phenomenon of accelerated convergence, one perspective which can be particularly intuitive is provided by interpreting optimisation algorithms as (discretisations of) dynamical systems. A recurring pattern is that while gradient descent `behaves like' a particle which follows the direction of steepest descent of $f$, the `optimal' algorithms which achieve improved convergence rates can often be viewed as kinetic particles, i.e. particles with a position and a momentum.

% To be more precise, \cite{wilson2016lyapunov} draw a connection between the fast gradient method of \citet{nesterov1983method} and the second-order ODE
% %
% \begin{align*}
%     \ddot{\theta}_{t} + \gamma\cdot\eta\cdot\dot{\theta}_{t} + \eta\cdot\nabla_{\theta}f\left(\theta_{t}\right) = 0,
% \end{align*}
% %
% where $\gamma,\eta$ are positive hyperparameters. When $f$ is a convex quadratic function, this ODE reproduces the dynamics of a damped harmonic oscillator \citep{mccall2010classical} , and this equips the hyperparameters of the ODE with intuitive interpretations: $\eta^{-1}$ represents the mass of the particle, and $\gamma$ determines the strength of the damping. Additionally, in the massless limit (i.e. sending $\eta \to \infty$ and rescaling time appropriately), one can formally recover the gradient flow ODE $\gamma\cdot\dot{\theta}_{t} + \nabla_{\theta} f\left(\theta_{t}\right) = 0$.

% One can equally re-write the same dynamics as a first-order system of ODEs by introducing the momentum variable $m=\eta^{-1}\cdot\dot{\theta}$, which yields
% %
% \begin{align*}
%     \dot{\theta}_{t} &=\eta\cdot m_{t} \\
%     \dot{m}_{t}	&=-\gamma\cdot\eta\cdot m_{t}-\nabla_{\theta}f\left(\theta_{t}\right).
% \end{align*}
% %
% Introducing the `Hamiltonian' function $F\left(\theta,m\right) :=f\left(\theta\right) + \frac{\eta}{2}\cdot\left\Vert m\right\Vert _{2}^{2}$, this system can be interpreted as a `damped' or `conformal' Hamiltonian flow for $F$ \citep{mclachlan2001conformal, maddison2018hamiltonian}, i.e.
% %
% \begin{align*}
%     \left(\begin{array}{c}
% \dot{\theta}_{t}\\
% \dot{m}_{t}
% \end{array}\right)=-\left(\begin{array}{cc}
% 0_{d} & -I_{d}\\
% I_{d} & \gamma\cdot I_{d}
% \end{array}\right)\cdot\nabla_{\left(\theta,m\right)}F\left(\theta_{t},m_{t}\right).
% \end{align*}
% %
% In this sense, the fast gradient method of Nesterov admits an interpretation as a discretisation of a damped Hamiltonian flow, corresponding to an augmented loss function.

% % Consider minimizing $f:\mathbb{R}^d \to \mathbb{R}$.
% % In machine learning, these problems are typically tackled using first-order methods such as gradient descent. However, gradient descent does not achieve optimal rates \citep{nemirovskij1983problem}, and momentum is often introduced to accelerate gradient descent \citep{nesterov1983method}.

% % One perspective of understanding momentum-based methods is via their continuous limits \citep{su2014differential}. In particular, \citet{wilson2016lyapunov} showed that the following ODE governs a class of accelerated algorithms in Euclidean spaces:
% % %
% % \begin{equation}
% % 	\ddot{\theta}_t + \gamma \eta \dot{\theta}_t + \eta \nabla_\theta f(\theta_t) = 0.
% % 	\label{eq:masterode}
% % \end{equation}
% % %
% % When $d=1$ and $f(\theta)=\frac{1}{2} \|\theta\|^2$, this ODE is the same as one modelling the behaviour of a damped harmonic oscillator \citep{mccall2010classical}. In this case, the parameters $\gamma$ and $\eta$ have intuitive interpretations: $\eta$ is the reciprocal of the mass and $\gamma$ determines the strength of the damping. It can be seen that \eqref{eq:masterode} recovers the gradient flow ODE in the massless limit, i.e., $\gamma \rightarrow \infty$.

% % %
% % The ODE \eqref{eq:masterode} can be equivalently written in an expanded space with a ``momentum'' variable, $m_t= \frac{1}{\eta} \dot{\theta}_t$, which gives rise to the following system of coupled  first-order ODEs:
% % %
% % \begin{align*}
% %   \dot{\tmo}_t &= - \gamma \eta m_t - \nabla_\theta f(\theta_t),& \quad \dot{\theta}_t &= \eta m_t.
% % \end{align*}
% % %
% % These dynamics can be more compactly written by introducing an augmented function $F(\theta, m) =f(\theta) + \frac{\eta}{2}\|m\|^2_2$, and defining the damped (or conformal \citep{mclachlan2001conformal}) Hamiltonian flow of $F$ \citep{maddison2018hamiltonian} as
% % %
% % $$
% % \begin{pmatrix}
% %     \dot{\theta}_t \\ \dot{\tmo}_t
% % \end{pmatrix}=
% % -\begin{pmatrix} 0_{d} & -I_{d}  \\
% %                     I_{d}  & \gamma I_{d} \end{pmatrix}
% % \nabla_{(\theta,\tmo)} F_t,
% % $$
% % % $$
% % % \begin{pmatrix}
% % %     \dot{\theta}_t \\ \dot{\tmo}_t
% % % \end{pmatrix}=
% % % -\begin{pmatrix} 0_{d} & -I_{d}  \\
% % %                     I_{d}  & \gamma I_{d} \end{pmatrix}
% % % \nabla_{(\theta,\tmo)} F(\theta_t,m_t),
% % % $$
% % % \adam{Is there a benefit to introducing $F_t$ rather than just substituting this expansion into the above eqn? Personally, that would seem clearer to me, and would reudce the notational burden.}
% % %
% % where $F_t := F(\theta_t, \tmo_t)$. Thus, we can interpret accelerated algorithms as a damped Hamiltonian flow of an augmented loss function.

% \subsection{Accelerating Gradient Descent in $\cal{P}(\mathbb{R}^d)$.}
% \label{sec:p_momentum}

% A remarkable insight of \citep{jordan1998variational} was to recognise a connection between the overdamped Langevin SDE and the geometry of the Wasserstein space of probability distributions. More precisely, for a fixed $p \in \mathcal{P}\left(\mathbb{R}^{d}\right)$, consider the diffusion process given by 
% %
% \begin{align*}
%     \mathrm{d}X_{t}=\nabla_{x}\log p\left(X_{t}\right)\,\mathrm{d}t+\sqrt{2}\,\mathrm{d}W_{t},
% \end{align*}
% %
% and write $q_{t}=\mathrm{Law}\left(X_{t}\right)$. Abusing notation to identify probability distributions with their density, $q_{t}$ satisfies the Fokker-Planck PDE
% %
% \begin{align*}
%     \partial_{t}q_{t}=\nabla_{x}\cdot\left(q_{t}\cdot\nabla_{x}\left(\log\left(\frac{q_{t}}{p}\right)\right)\right).
% \end{align*}
% \jl{Im tempted to remove the inner two brackets}
% %
% A major insight of \citep{jordan1998variational} was to note that the drift term on the right-hand side of this PDE admits an interpretation as a gradient in the Wasserstein space. Specifically, defining $\mathcal{E}_{p}\left(q\right) := \mathsf{KL} \left( q, p \right)$, they observed that
% %
% \begin{align*}
%     \nabla_{x}\cdot\left(q\cdot\nabla_{x}\left(\log\left(\frac{q}{p}\right)\right)\right)=-\nabla_{W}\mathcal{E}_{p}\left(q\right),
% \end{align*}
% %
% and hence that the Fokker-Planck PDE can be interpreted as a gradient flow on the space of probability distributions. This connection has inspired a great deal of follow-up work, see CITE CITE CITE.

% Viewing the overdamped Langevin SDE as a sort of `gradient descent on probability space', and recalling that gradient descent can often be improved upon by `momentum-type' schemes, a natural question is whether the same intuition might enable the development of accelerated diffusion processes for sampling. In particular, in the same way that the gradient flow of $\mathcal{E}_{p}$ gives rise to an evolution of distributions which can be interpreted as the solution to the Langevin SDE, might a damped Hamiltonian flow of a related functional correspond to some other SDE with a `momentum' interpretation?

% This question was answered in the affirmative by \cite{ma2019there}, who show that this damped Hamiltonian flow on probability space corresponds directly to the \textit{underdamped} Langevin SDE. More precisely, let $\eta>0$, and consider the probability distribution on $\mathbb{R}^{d}\times\mathbb{R}^{d}$ given by the product of $p\left(x\right)$ with a Gaussian distribution over `momentum' variables $\mathcal{N}\left(u\mid0,\eta^{-1}\cdot I_{d}\right)$. Defining $\mathcal{F}:\mathcal{P}\left(\mathbb{R}^{d}\times\mathbb{R}^{d}\right)\to\mathbb{R}$ by
% %
% \begin{align*}
%     \mathcal{F} \left(q\right) = \mathsf{KL}\left(q\left(x,u\right), p\left(x\right) \cdot \mathcal{N}\left(u\mid0,\eta^{-1}\cdot I_{d}\right)\right),
% \end{align*}
% %
% the authors construct the damped Hamiltonian flow of $\mathcal{F}$ with respect to the 2-Wasserstein geometry on $\mathcal{P}\left(\mathbb{R}^{d} \times \mathbb{R}^{d}\right)$, and show that the resulting evolution of probability distributions can be interpreted in terms of the underdamped Langevin SDE
% %
% \begin{align*}
%     \mathrm{d}X_{t}	&=\eta\cdot U_{t}\,\mathrm{d}t \\
%     \mathrm{d}U_{t} &=\nabla_{x}\log p\left(X_{t}\right)\,\mathrm{d}t-\gamma\cdot\eta\cdot U_{t}\,\mathrm{d}t+\sqrt{2\cdot\gamma}\,\mathrm{d}W_{t}.
% \end{align*}
% %

% % The path $q_t := \rm{Law}(X_t)$ of the (overdamped) Langevin SDE, $dX_t = \nabla\log p(X_t)dt + \sqrt{2}dW_t$, can be viewed as gradient descent on the functional $f(q) := \rm{KL}(q|p): \cal{P}(\mathbb{R}^d) \rightarrow \bb{R}$ where the gradient is prescribed by the Wasserstein-$2$ distance \citep{jordan1998variational}. This can be seen from its Fokker-Planck equation, namely, we have
% % $$
% % \dot{q}_t = \nabla_x \cdot \left [q_t \nabla_x \log \frac{q_t}{p} \right ] = - \nabla_W f.
% % $$
% % A natural question is whether we can accelerate the (overdamped) Langevin SDE by constructing an associated damped Hamiltonian flow for an augmented loss function (similarly to the Euclidean case as see in \Cref{sec:euclidean_momentum}). \citet{ma2019there} answered this question in the affirmative and showed that incorporating momentum in the vector field led to dynamics equivalent to those of the familiar \emph{underdamped} Langevin SDE. More specifically, consider the augmented function is $F:q \mapsto \rm{KL}(q|p(x)p(\qmo)); \cal{P}(\bb{R}^d \times \bb{R}^d) \rightarrow \mathbb{R}$ where $p(\qmo)=\cal{N}(0,\eta^{-1}I)$ with it's damped Hamiltonian flow  given by
% % $$
% % \begin{pmatrix}
% % 	\dot{x}_t \\ \dot{\qmo}_t
% % \end{pmatrix}= - \begin{pmatrix} 0_{d} & -I_{d}  \\
% % 	I_{d}  & \gamma I_{d} \end{pmatrix}
% % \nabla_{(x, \qmo)} \delta_q F[q](x_t, \qmo_t),
% % $$
% % where the first variation is given by $\delta_q F[q] (x, \qmo) = \log \frac{q(x, \qmo)}{p(x, \qmo)}$ \citep{ma2019there}. The aforementioned flow is equivalent to the underdamped Langevin SDE:
% % \begin{align*}
% % 	dX_t &= \eta \Qmo_t dt \\
% % 	d\Qmo_t &= \nabla_x \log p(x)dt - \gamma \eta \Qmo_tdt + \sqrt{2\gamma} dW_t.
% % \end{align*}
% % %
% % \begin{remark*}[``Equivalence'' between ODE and SDE]
% % The relationship between above ODE and SDE is that they share the same evolution of the marginal density, i.e., $\partial_t p_t(x) = \partial_t q_t(x)$ where $p_t = \rm{Law}(x_t)$, and $q_t = \rm{Law}(X_t)$, and so the marginals of both processes are the same given the same initial conditions (for instance, see \Cref{sec:ula_sde}). Note that $x_t$ is a random variable where the randomness is induced from the initial point $x_0 \sim p_0$. However, they ($X_t$ and $x_t$) typically do not share the same path-wise properties. For the remainder of the manuscript, we will say that $x_t$ (described by an ODE) is equivalent to $X_t$ (governed by a SDE) when the evolution of their density is the same. Their relationship in the context of sampling can be found in \citet{maoutsa2020interacting}.
% % \end{remark*}

% Note that there are various routes which one could pursue here: our original gradient flow is an evolution on $\left(\theta,q\right) \in \mathbb{R}^{d_{\theta}} \times \mathcal{P}\left(\mathbb{R}^{d_{x}}\right)$, and so we can choose to i) accelerate the evolution of $\theta$, by introducing a momentum variable $m\in\mathbb{R}^{d_{\theta}}$, ii) accelerate the evolution of $q$, by working with $\tilde{q}\in\mathcal{P}\left(\mathbb{R}^{d_{x}}\times\mathbb{R}^{d_{x}}\right)$ (equivalently, instead of considering the evolution of a standard particle $x\in\mathbb{R}^{d_{x}}$, consider the evolution of a kinetic particle $\left(x, u\right) \in \mathbb{R}^{d_{x}} \times \mathbb{R}^{d_{x}}$, or iii) both of these at once. We take the third route in what follows, noting that the first two routes can be obtained as different degenerate limits of the third.

% To this end, we introduce the augmented joint target $\rho_{\theta}\left(x,u\right) := p_{\theta}\left(y,x\right) \cdot p_{U}\left(u\right)$, where $p_{U} \left(u\right) = \mathcal{N}\left(u\mid0,\eta_{x}^{-1}\cdot I_{d_{x}}\right)$, as well as the augmented free energy functional
% %
% \begin{align*}
%     \mathcal{F}\left(\theta,m,q\right):=\int q\left(x,u\right)\cdot\log\left(\frac{q\left(x,u\right)}{\rho_{\theta}\left(x,u\right)}\right)\,\mathrm{d}x\,\mathrm{d}u+\frac{\eta_{\theta}}{2}\cdot\left\Vert m\right\Vert _{2}^{2}.
% \end{align*}
% %
% The $\left(\gamma_{\theta},\gamma_{x}\right)$-damped Hamiltonian flow of $\mathcal{F}$ then takes the form
% %
% \begin{align*}
%     \left(\begin{array}{c}
% \dot{\theta}_{t}\\
% \dot{m}_{t}
% \end{array}\right)=-\left(\begin{array}{cc}
% 0_{d_{\theta}} & -I_{d_{\theta}}\\
% I_{d_{\theta}} & \gamma_{\theta}\cdot I_{d_{\theta}}
% \end{array}\right)\cdot\nabla_{\left(\theta,m\right)}\mathcal{F}\left(\theta,m,q\right)
% \end{align*}
% %
% for the `parameter-space' variables, and
% %
% \begin{align*}
%     \left(\begin{array}{c}
% \dot{x}_{t}\\
% \dot{u}_{t}
% \end{array}\right)=-\left(\begin{array}{cc}
% 0_{d_{x}} & -I_{d_{x}}\\
% I_{d_{x}} & \gamma_{x}\cdot I_{d_{x}}
% \end{array}\right)\cdot\nabla_{\left(x,u\right)}\delta_{q}\mathcal{F}\left(\theta,m,q\right).
% \end{align*}
% %
% Again deferring technical details to the appendix, this admits an interpretation via the dynamics
% %
% \begin{align*}
%     \mathrm{d}\theta_{t}	&=\eta_{\theta}\cdot m_{t}\,\mathrm{d}t \\
% \mathrm{d}m_{t}	&=-\gamma_{\theta}\cdot\eta_{\theta}\cdot m_{t}\,\mathrm{d}t+\int q_{t}\left(\mathrm{d}x,\mathrm{d}u\right)\cdot\nabla_{\theta}\ell\left(\theta_{t},x\right)\,\mathrm{d}t \\
% \mathrm{d}x_{t}	&=\eta_{x}\cdot u_{t}\,\mathrm{d}t \\
% \mathrm{d}u_{t}	&=-\gamma_{x}\cdot\eta_{x}\cdot u_{t}\,\mathrm{d}t+\nabla_{\theta}\ell\left(\theta_{t},x_{t}\right)\,\mathrm{d}t+\sqrt{2\cdot\gamma_{x}}\,\mathrm{d}W_{t} \\
% \text{where}\quad q_{t}	&=\mathrm{Law}\left(x_{t},u_{t}\right);
% \end{align*}
% %
% this can then be converted into an implementable particle algorithm in a similar vein to PGD (though some care is required in order to obtain an accelerated convergence rate; see Section XXX). We refer to the resulting procedure as APGD (might recommend momentum PGD?).

% Inspired by prior works as outlined in \Cref{sec:euclidean_momentum,sec:p_momentum}, accelerating gradient flows amounts to constructing an extended damped Hamiltonian system incorporating momentum. In this section, we propose the damped Hamiltonian flow to accelerate the gradient flow of  \texttt{PGD}. To this end, we construct the augmented joint target $\rho_\theta(x, {\qmo}) := p_\theta(y, x) p_\Qmo ({\qmo})$ with $p_\Qmo =\mathcal{N}\left (0, {\eta_x^{-1}} I_{d_x} \right )$, and we define the augmented free energy $\cal{F}: \mathbb{R}^{d_\theta} \times \mathbb{R}^{d_\theta} \times \mathcal{P}(\mathbb{R}^{d_x} \times \mathbb{R}^{d_x}) \rightarrow \mathbb{R}$ as
% \begin{align}
%     \mathcal{F}(\theta, m, q) &:= \int \log \frac{q(x,{\qmo})}{\rho_\theta(x, {\qmo})} q(dx\times d{\qmo}) + \frac{\eta_\theta }{2} \| m \|^2,
%     \label{eq:aug_F}
% \end{align}
% where $\eta_x, \eta_\theta > 0$, and the momentum variable $\tmo$ and $\qmo$ are associated with parameter $\theta$ and variable $x$, respectively. We propose the damped Hamiltonian flow of the augmented free energy $\cal{F}$ given by
% \begin{align}
% \begin{pmatrix}
%     \dot{\theta}_t \\
%     \dot{\tmo}_t
% \end{pmatrix}
%  &= -\begin{pmatrix} 0_{d_\theta} & -I_{d_\theta} \\
%                     I_{d_\theta} & \gamma_\theta I_{d_\theta}
%     \end{pmatrix}
%     \nabla_{(\theta, \tmo)} \cal{F}_t, \quad 
% \begin{pmatrix}
%     \dot{x}_t \\
%     \dot{\qmo}_t
% \end{pmatrix}
%  = - \begin{pmatrix}
%         0_{d_x}  & -I_{d_x} \\
%         I_{d_x} & \gamma_x I_{d_x}
%     \end{pmatrix}
%         -\nabla_{(x, \qmo)} \delta_{q} \cal{F}_t,
% \end{align}
% %
% where $\gamma_\theta, \gamma_x > 0$; $\cal{F}_t = \cal{F}(\theta_t, m_t, q_t)$ and the first variation of $\cal{F}_t$ is given by $\delta_q \cal{F}_t =  \log \frac{q_t}{ \rho_{\theta_t}}$ (see \Cref{prop:fv}). More specifically, for continuous time $\texttt{APGD}$, we have
% %
% \begin{subequations}
% 	\label{eq:aflow}
% 	\begin{align}
% 			d{\theta}_t &= \eta_\theta m_t \, dt,\\
% 			d{\tmo}_t &= \left [\int \nabla_\theta \ell (\theta_t, x) q_t(dx) \right ]\,dt-  \gamma_\theta \eta_\theta m_t\, dt, \label{eq:aflow_tmo}\\
% 			q_t = \rm{Law}(x_t) : d{x}_t &= \eta_x {\qmo}_t\, dt,\\
% 			d{\qmo}_t
% 			&=
% 			\nabla_x \ell ({\theta_t}, x_t)\,dt - \gamma_x \eta_x {\qmo}_t\,dt - \gamma_x \nabla_{\qmo} \log {q_t(x_t, {\qmo}_t)} \,dt
% 			\label{eq:aflow_qmo}.
% \end{align}
% \end{subequations}
% %

% %
% The choice of hyperparameters ${\eta_x, \eta_\theta, \gamma_x, \gamma_\theta}$ plays a crucial role in \texttt{APGD}. In \Cref{eq:different_regimes}, we show that there are three different regimes that arises from the choice in hyperparameters: underdamped, overdamped, and critically damped. In the underdamped regime, the parameter quickly approaches the true point, but will oscillate around it before converging later. One migrating trick is to restart the momentum is using adaptive restart methods \citep{o2015adaptive}. In the overdamped case, the \texttt{APGD} behaves similarly to $\texttt{PGD}$. However, the most desirable case is the critically damped case, where the parameter rapidly approaches the true point without oscillation. Unfortunately, obtaining hyperparameters that satisfy this regime is difficult, and we leave for future work.



% In this section, we study the convergence properties of the flow described in \eqref{eq:aflow}. Following the work of \citet{wilson2016lyapunov, ma2019there, wibisono2016variational}, we will use \citet{lyapunov1992general}'s method  to analyse the convergence of the continuous process. It is based upon a simple idea of constructing a positive definite function $\mathcal{L}$ such that it decreases along the trajectory of a dynamical system. The existence of a Lyapunov function guarantees that the system convergence and approaches a region where the Lyapunov function $\mathcal{L}$ is minimized.

% First consider how the free energy $\cal{F}$ evolves with time. Explicitly, we can see that its time derivative is given by:
% $$
% \dot{\cal{F}}_t = -\gamma_\theta \|\nabla_{m}\cal{F}_t\|^2  -  \gamma_x\|\nabla_{\qmo}\delta_{q}\cal{F}_t\|^2_{q_t}\le 0.
% $$
% %
% See \Cref{prop:contraction} for the calculations. This only assures us that the $\cal{F}$ is non-increasing in time and does not establish convergence of $\cal{F}$ to a minimizer. This is due to the fact that the gradient... . In order to establish convergence, we follow in \cite{wilson2016lyapunov, ma2019there} and propose to study following Lyapunov function that upper bounds $\cal{F}$: 
% %
% \begin{equation}
% 	\label{eq:lya_def}
% \mathcal{L} :=\cal{F}
% 	+\log p_{\theta_*}(y)
% 	+\iprod{\nabla_{(\theta, \tmo)} \cal{F}}{T_{(\theta,\tmo)} \nabla_{(\theta, \tmo)} \cal{F}}
% 	+\iprod{\nabla_{(x,\qmo)} \delta_q \cal{F}}{T_{(x,\qmo)}\nabla_{(x,\qmo)}\delta_q \cal{F}}_q,
% \end{equation}
% where $T_{(\theta,\tmo)}$ and $T_{(x,\qmo)}$ are positive semi-definite matrices that are defined as
% %
% {
% \renewcommand*{\arraystretch}{1.25}
% \begin{align}
% 	T_{(\theta,\tmo)}
% 	:= \frac{1}{K}
% 	\begin{pmatrix}
% 		\tau_\theta I_{d_\theta} & \frac{\tau_{\theta \tmo}}{2} I_{d_\theta} \\
% 		\frac{\tau_{\theta \tmo}}{2} I_{d_\theta}  & \tau_{\tmo} I_{d_\theta}
% 	\end{pmatrix},\quad 
% 	T_{(x,\qmo)}
% 	:=\frac{1}{K}
% 	\begin{pmatrix}
% 		\tau_x I_{d_x} & \frac{\tau_{x \qmo}}{2} I_{d_x} \\
% 		\frac{\tau_{x \qmo}}{2} I_{d_x}  & {\tau_{\qmo}}  I_{d_x}
% 	\end{pmatrix}
% \end{align}
% }
% %
% In \Cref{prop:convergence_flow},  we establish sufficient conditions for $\cal{L}_t$ to decay exponentially in time, and thus convergence of the flow of $\cal{F}$. The convergence is established under a gradient dominance criterion, called log-Sobolev inequality (see \Cref{ass:logsobolev}), which is a natural extension to the Polyak-Łojasiewicz Inequality for the Euclidean gradient flows \citep{polyak1964gradient} and the log-Sobolev inequality of Wasserstein flows \citep{gross1975logarithmic}.
% %
% \begin{proposition}[Exponential  Convergence of the Continuous Flow]
% 	\label{prop:convergence_flow}
% 	Under the $K$-Lipschitz gradient \Cref{ass:gradlip} and the log-Sobolev \Cref{ass:logsobolev} with constant $C_{\cal{E}}$, given parameters $\gamma_x, \gamma_\theta, \eta_x, \eta_\theta$ if there exists constants $\tau_\theta, \tau_{\theta \tmo}, \tau_\tmo, \tau_x, \tau_{x\qmo},\tau_\qmo$ such that inequalities in \eqref{eq:flow_conditions} are satisfied, we have
%     $$
% 	\dot{\mathcal{L}}_t \le - \frac{C_{\cal{E}}}{10}\mathcal{L}_t.
%     $$
%     Moreover, we have exponential convergence of $\cal{F}_t$
%     $$
%     \mathcal{F}_t + \log p_{\theta_*} \le \mathcal{L}_0\exp \left ( - \frac{C_{\cal{E}}}{10}t \right ).
%     $$
% \end{proposition}
% %
%  For the sake of brevity, the proof and inequalities is deferred to \Cref{sec:convergence_flow}. For concreteness, we show example hyperparamters for which inequalities of \eqref{eq:flow_conditions} are satisfied in \ref{sec:eq_flow_conditions true}. 
% %


% % % % 

DISCRETISATION

In order to realize an actionable algorithm, we need to discretize the dynamics \eqref{eq:aflow} in time so that they may be simulated. However, directly discretizing \eqref{eq:aflow} is intractable due to the need to evaluate the integral w.r.t.\ $q_t$ in \eqref{eq:aflow_tmo}, and the score of $q_t$ \eqref{eq:aflow_qmo}. In this section, we circumvent these issues by deriving a flow which approximates \eqref{eq:aflow}, then we propose a discretization of the approximate flow \eqref{eq:aflow} to obtain an accelerated algorithm.

To bypass the intractability of the score in \eqref{eq:aflow_tmo}, we identify the equivalent stochastic dynamics driven by Brownian motion (written as a Stochastic Differential Equation (SDE)) that does not require knowledge of the score. More specifically, we can
equivalently write the flow of $(x_t, \qmo_t)$ as solving the following McKean-Vlasov SDE (see \Cref{sec:ula_sde}):
%
\begin{align*}
	d{X}_t &= \eta_x {\Qmo}_t dt, \\
	d{\Qmo}_t &= \nabla_x \ell (\theta_t, X_t)dt - \gamma_x \eta_x {\Qmo}_tdt + \sqrt{2\gamma_x} dW_t,
\end{align*}
%
where $W_t$ denotes Brownian motion.
This SDE is equivalent to \eqref{eq:aflow} in the sense that they share the same Fokker-Planck equation. Unsurprisingly, like in the sampling case \citep{ma2019there}, this SDE corresponds to the underdamped Langevin SDE.
If we can simulate from the SDE, then we can approximate the integral in \eqref{eq:aflow_tmo} using a particle approximation of $q_t$. To be precise, an $N$-particle $\{X^i_t\}_{i=1}^N$ approximation of $q_t$ is given by $q_t \approx \frac{1}{N} \sum_{i=1}^N \delta_{X^i_t}$ where $X^i_t$ solves
%
\begin{align*}
\forall i \in [N] : d{X}^i_t &= \eta_x {\Qmo}^i_t dt, \\
\forall i \in [N] : d{\Qmo}^i_t &= \nabla_x \ell (\theta_t, X_t^i)dt - \gamma_x \eta_x {\Qmo}^i_tdt + \sqrt{2\gamma_x} dW^i_t,
\end{align*}
and $\{W^i_t\}_{i=1}^M$ denotes $N$ independent Brownian motions.
%
Given such an approximation, we can approximate the integral \eqref{eq:aflow_tmo} with $\int \nabla_\theta \ell (\theta_t, x_t) q_t(x_t)dx \approx \frac{1}{N}\sum_{i=1}^N \nabla_\theta \ell (\theta_t, X_t^i)=: \nabla_\theta \hat{\cal{F}}(\theta_t, \{X_t^i\}_{i=1}^{M})$. In summary, we have the following approximation to the flow \eqref{eq:aflow} written as a McKean-Vlasov SDE:
\begin{subequations}
	\begin{align}
	           d{\theta}_t &= \eta_\theta m_t \, dt,\\
		   d{\tmo}_t &= \left [\frac{1}{N}\sum_{i=1}^N \nabla_\theta \ell (\theta_t, X_t^i) \right ]\,dt-  \gamma_\theta \eta_\theta m_t\, dt, \\
\forall i \in [N]: d{X}^i_t &= \eta_x {\Qmo^i_t} dt, \\
\forall i \in [N]: d{\Qmo}^i_t &= \nabla_x \ell (\theta_t, X_t^i)dt - \gamma_x \eta_x {\Qmo_t^i}dt + \sqrt{2\gamma_x} dW^i_t.
 	\end{align}
	\label{eq:aaflow}
\end{subequations}
%
We are now ready to discretize the flow in time. Direct Euler-Maruyama discretization (see \eqref{eq:aflow-em}\adam{Dangling reference.} in the Appendix), as shown in \Cref{fig:dont_use_em}, does not result in an accelerated algorithm. However, other schemes can produce accelerated algorithms. In this work, we propose a new scheme that is inspired by \citet{cheng2018underdamped} and \citet{sutskever2013importance}'s interpretation of \citet{nesterov1983method}.

Following in the style of \citep{cheng2018underdamped}, given $(\theta_0, m_0, \{(X^i_0, U_0^i)\}_{i=1}^N)$, we consider the following approximating SDE of the single step transition for time $t\in [0, h]$ of \eqref{eq:aaflow}:
%
\begin{subequations}
	\label{eq:aaaflow}
	\begin{align}
		d\tilde{\theta}_t &= \eta_\theta \tilde{m}_t \, dt,\\
		d\tilde{\tmo}_t &= \left [\frac{1}{N}\sum_{i=1}^N \nabla_\theta \ell (\theta_0 + \omega_\theta (h) m_0, X_0^i) \right ]\,dt-  \gamma_\theta \eta_\theta \tilde{m}_t\, dt \label{eq:transition_sde_tmo},\\
\forall i \in [N]: 		d\tilde{X}^i_t &= \eta_x {\tilde{\Qmo}^i_t} dt, \\
\forall i \in [N]: 		d\tilde{\Qmo}^i_t &= \nabla_x \ell (\tilde{\theta}_h, X_0^i)dt - \gamma_x \eta_x \tilde{\Qmo}_tdt + \sqrt{2\gamma_x} dW^i_t, \label{eq:transition_sde_qmo}
	\end{align}
\end{subequations}
where $\omega_\theta(t) = \exp (- \eta_\theta \gamma_\theta t)$.
This is a linear non-homogenous SDE that we can solve analytically (see \Cref{sec:our_discretization} for details).
In summary, for small step $h>0$, we arrive at the following iteration $\forall i \in [N]$:
%
\begin{subequations}
	\begin{align*}
		\tilde{\theta}_{k+1} &= \tilde{\theta}_k + \frac{1}{\gamma_\theta} \left [ (1-\omega_\theta(h))\tilde\tmo_k + \left (h - \frac{1-\omega_\theta(h)}{\gamma_\theta \eta_\theta}\right )\nabla_\theta \hat{\cal{F}}(\tilde{\theta}_k + \omega(h)\tilde{m}_{k}, \{\tilde{X}_k^i\}_{i=1}^M) \right ]\\ 
		\tilde{\tmo}_{k+1} &= \omega_\theta (h) \tilde{\tmo}_k + \frac{1- \omega_\theta(h)}{\gamma_\theta \eta_\theta} \nabla_\theta \hat{\cal{F}}(\tilde\theta_k + \omega_\theta(h)\tilde{\tmo}_k, \{\tilde{X}_k^i\}_{i=1}^M)\\
		\forall i \in [N]: \tilde{X}^i_{k+1} &= \tilde{X}_k^i + \frac{1}{\gamma_x} \left [ ( 1- \omega_x (h))  \tilde{\Qmo}^i_k +  \left ( t - \frac{1-\omega_x (h)}{\gamma_x\eta_x} \right ) \nabla_x \ell (\tilde{\theta}_{k+1}, \tilde{X}_k^i) \right ] + L_\Sigma^{XX} \xi_k^i, \\
		\forall i \in [N]: \tilde{\Qmo}^i_{k+1} &= \omega_x (h) \tilde{\Qmo}^i_k +  \frac{1-\omega_x (h)}{\gamma_x\eta_x}\nabla_x \ell (\tilde{\theta}_{k+1}, \tilde{X}^i_k) + L_\Sigma^{X \Qmo} \xi_k^i + L_\Sigma^{\Qmo\Qmo}\xi_k^{i'}.
	\end{align*}
\end{subequations}
%
where $\omega_x(t) := \exp(-t\gamma_x\eta_x)$; $\xi^i_k, \xi'^i_k \sim \mathcal{N}(0_{d_x}, I_{d_x})$; and the constants $L^{XX}_\Sigma$, $L^{X\Qmo}_\Sigma$, and $L^{\Qmo\Qmo}_\Sigma$ whose definitions can be found in Appendix, see \Cref{eq:sampling_constants}. The constants are derived from the Cholesky decomposition of the transition covariance matrix to ensure that $\tilde{X}^i_{k+1}$ and $\tilde{\Qmo}^i_{k+1}$ have the correct covariance structure. 

The key difference between the discretization of \citet{cheng2018underdamped} and ours is that our proposed approach includes additional terms in the gradient terms of \eqref{eq:transition_sde_tmo} and \eqref{eq:transition_sde_qmo}. Similar to \citet{sutskever2013importance}'s NAG, \adam{what?}

Another natural scheme is using a combination of \citet{nesterov1983method} and \citet{cheng2018underdamped} for the $\theta_t$ and $q_t$ respectively. For brevity, we differ the derivation and resulting algorithm to the \Cref{sec:nc_nag}, and compare its performance with our proposed discretization in \Cref{sec:experiments}.

% % % % % 


%At least in the abstract, one can consider following a similar program for solving optimisation problems over the space of probability distributions on Euclidean space, $\mathcal{P} \left( \mathbb{R}^d \right)$. One challenge in making this idea practical is how to endow this space with a suitable geometric structure compatible with relevant algorithmic primitives. That is, when considering functionals $\mathcal{F} : \mathcal{P} \left( \mathbb{R}^d \right) \to \mathbb{R}$ and distributions $q, \tilde{q}$ which are `close' to one another in a relevant sense, we want to be able to make estimates of the form
%
%$    \mathcal{F} \left( \tilde{q} \right) \approx \mathcal{F} \left( q \right) + \mathrm{D} \mathcal{F} \left [q \right] \left( \tilde{q} - q \right),$
%
%for some suitable notion of derivative $\mathrm{D} \mathcal{F}$. In our work, we consider the geometry induced by the Wasserstein-2 metric \citep{jordan1998variational}. Other choices for distances will generate different geometries and algorithms, e.g., the Stein geometry \citep{duncan2019geometry, liu2017stein, sharrock2023coinem}.

%The important objects are then as follows: given a functional $\mathcal{F} : \mathcal{P} \left( \mathbb{R}^d \right) \to \mathbb{R}$ and distributions $q, \tilde{q} \in \mathcal{P} \left( \mathbb{R}^d \right)$, define the functional gradient of $\delta_q \cal{F} : \mathcal{P} \left( \mathbb{R}^d \right) \to \left( \mathbb{R}^d \to \mathbb{R} \right)$ so that
%
%$    q \approx \tilde{q} \implies \mathcal{F} \left( \tilde{q} \right) \approx \mathcal{F} \left( q \right) + \int \delta_q \cal{F} \left[ q \right] \left( x \right) \, \left( \tilde{q} \left( x \right) - q \left( x \right) \right) \, \mathrm{d} x.$
%
%Now, let $v$ denote a vector field, let $\epsilon > 0$, and write $q_\epsilon$ for the law of $x + \epsilon v \left( x \right)$ when $x \sim q$. Under suitable assumptions, one can then compute that
%
%$    \mathcal{F} \left( q_\epsilon \right) = \mathcal{F} \left( q \right) + \epsilon \int q \left( \mathrm{d}x \right) \left\langle \nabla_x \delta_q \cal{F} \left[ q \right] \left( x \right), v \left( x \right) \right\rangle + o \left( \epsilon \right)$ $\text{as } \epsilon \to 0^+$, where $\iprod{\cdot}{\cdot}$ is the  Euclidean inner product \citep[Lemma 10.4.1]{ambrosio2005gradient}.
%
%Therefore, the Wasserstein gradient of $\mathcal{F}$ is defined as
%
%$    \nabla_{\sf{W}} \mathcal{F} \left( q \right) = - \nabla_x \cdot \left( q \nabla_x \delta_q \cal{F} \left [ q \right ] \right).$
%
%Interpreting gradients from the perspective of steepest descent, this expression reflects the notion that in order to reduce $\mathcal{F} \left( q \right)$ by updating $q$ by a perturbation which is small in the sense of the Wasserstein-2 (denoted by $\sf{W}_2$) geometry, it would be suitable to take each $x$ in the support of $q$ and transport it towards $x - \epsilon \nabla_x \delta_q \cal{F} \left[ q \right] \left( x \right)$ (for more details, see \Cref{appen:gf_w2}).
